Learning Mixture Structure on Multi-Source Time Series for Probabilistic Forecasting

In many data-driven applications, collecting data from different sources is increasingly desirable for enhancing performance. In this paper, we are interested in the problem of probabilistic forecasting with multi-source time series. We propose a neural mixture structure-based probability model for learning different predictive relations and their adaptive combinations from multi-source time series. We present the prediction and uncertainty quantification methods that apply to different distributions of target variables. Additionally, given the imbalanced and unstable behaviors observed during the direct training of the proposed mixture model, we develop a phased learning method and provide a theoretical analysis. In experimental evaluations, the mixture model trained by the phased learning exhibits competitive performance on both point and probabilistic prediction metrics. Meanwhile, the proposed uncertainty conditioned error suggests the potential of the mixture model's uncertainty score as a reliability indicator of predictions.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

BIBLATEXFILES= $(wildcard *.bbx) $(wildcard *.cbx) $(wildcard *.dbx) $(wildcard *.lbx)
SAMPLEBIBLATEXFILES=$(patsubst %,samples/%,$(BIBLATEXFILES))

all:  ${PDF} ALLSAMPLES

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES: $(SAMPLEBIBLATEXFILES)
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/abbrev.bib: ACM-Reference-Format.bst
	perl -pe 's/MACRO ({[^}]*}) *\n/MACRO \1/' ACM-Reference-Format.bst \
	| grep MACRO | sed 's/MACRO {/@STRING{/' \
	| sed 's/}  *{/ = /' > samples/abbrev.bib 


samples/%.bbx: %.bbx
samples/%.cbx: %.cbx
samples/%.dbx: %.dbx
samples/%.lbx: %.lbx

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-sigconf-biblatex.pdf: samples/sample-sigconf-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-acmsmall-biblatex.pdf: samples/sample-acmsmall-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut \
	samples/*.run.xml samples/*.bcf $(SAMPLEBIBLATEXFILES)


clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

Version 1.84   Support for BibLaTeX rewritten (thanks to
	       Roberto Di Cosmo and Kartik Singhal)
	       Corrected German translation (thanks to Dirk Beyer)
	       New journals

Version 1.83   Support for multilanguage papers
	       ISSN changes for some journals

Version 1.82   Bug fixes.
	       New command \anon for anonymization of short strings.
	       Documentation update.

Version 1.81   Bug fixes
	       New bib field distinctURL to print URL even if doi is present.
	       Reworded samples

Version 1.80   New journals: DLT, FAC

Version 1.79   Fixed pages with index
	       (https://github.com/borisveytsman/acmart/issues/440)
	       Updated information for TAP, TCPS, TEAC

Version 1.78   Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.

Version 1.77   Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.76   Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.75   \country is now obligatory for addresses.
	       Added \AtBeginMaketitle

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.63a   Moved TQUANT to TQC

Version 1.63	New journals: TQUANT, FACMP

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.52    Another rewording of licenses

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.49    New jorunal:  DTRAP

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.47    New journal: THRI

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.43    Bug fixes

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.41    Rearranged bib files
                Added new badges

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.39    Added \authornotemark commmand

Version 1.38    Increase default font size for SIGPLAN

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

Version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

Version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

Version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

Version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

Version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

Version 1.28    Bug fixes: natbib=false now behaves correctly.

Version 1.27    Bug fixes

Version 1.26    Bug fixes

Version 1.25    Updated PACMPL journal option.

Version 1.24    Added IMWUT journal option.

Version 1.23    Added PACM PL journal option.

Version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

Version 1.21    Bibliography changes: added arXiv, some cleanup

Version 1.20    Bug fixes, documentation updates

Version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

Version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.


Version 1.17    Formatting changes for margins and lists.  Bug fixes.

Version 1.16    Formatting changes for headers and footers.

Version 1.15    New structured affiliation command.
                New commands for acknowledgements.

Version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

Version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

Version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

Version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

Version 1.10    Bug fixes

Version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

Version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes


==> backup.tex <==


% % ------------------------
% \begin{table*}[!htbp]
% \centering
% \caption{
% Point prediction performance of the mixture models by different training methods (mean and standard errors in two rows).
% The best results are marked in dark grey boxes.
% }
% \resizebox{0.5\textwidth}{!}{
% \begin{tabular}{l|ll|ll}
% \toprule       
%               & \multicolumn{2}{c|}{RMSE $\downarrow$}                                    & \multicolumn{2}{c}{MAE $\downarrow$} \\
%               & \multicolumn{2}{c|}{Share}       & \multicolumn{2}{c}{Share}  \\
%     Dataset    & Direct & Phased                  & Direct & Phased          \\
%     \midrule
%     \midrule
%     Site 0  & 27.173 & \best{19.022}         & 14.905 & \best{10.297} \\
%             & 1.617  & 0.054                 & 0.423  & 0.048         \\
%     \midrule
%     Site 1  & 41.549 & \best{18.517}         & 17.876 &\best{9.929}   \\
%             & 2.013  & 0.086                 & 1.102  & 0.027         \\
%     \midrule
%     Site 2  & 17.279 & \best{17.081}         & 8.832 & \best{8.573}   \\
%             & 0.021  & 0.087                 & 0.011 & 0.037          \\
%     \midrule
%     Site 3  & 30.509 & \best{21.969}         & 14.241 & \best{11.293}  \\
%             & 1.132  & 0.101                 & 0.102  & 0.059          \\
%     \midrule
%     Site 4  & 26.592 & \best{19.637}         & 17.908 & \best{10.638}  \\
%             & 1.123  & 0.062                 & 0.812  & 0.084          \\
%     \midrule
%     Site 5  & 30.233 & \best{20.578}         & 19.843 & \best{10.318}  \\
%             & 1.932  & 0.128                 & 1.324  & 0.049          \\
%     \midrule
%     Site 6  & 24.004 & \best{17.625}         & 22.274 & \best{8.631}   \\
%             & 1.433  & 0.063                 & 1.322  & 0.027          \\
%   \midrule
%     Site 7  & 22.654 & \best{19.887}         & 15.551 & \best{10.411}  \\
%             & 1.121  & 0.122                 & 1.143  & 0.059          \\
%     \midrule
%     Site 8  & 69.885 & \best{19.481}          & 18.619 & \best{10.025} \\
%             & 2.954  & 0.110                  & 1.232  & 0.029         \\
%     \midrule
%     Site 9  & 53.530 & \best{18.586}         & 25.555 & \best{10.178}   \\
%             & 2.132  & 0.034                 & 1.323  & 0.020           \\
%     \midrule
%     Site 10 & 28.426 & \best{19.072}         & 32.878 & \best{9.999}   \\
%             & 2.434  & 0.247                 & 1.232  & 0.033           \\
%     \midrule
%     Site 11 & 87.015 & \best{23.197}        & 18.667 & \best{11.036}  \\
%             & 2.545  & 0.137                & 1.345  & 0.042          \\
%     \midrule        
%     \midrule
%     Exc. A  &  & \best{}       &  & \best{} \\
%             &  &               &  &      \\
%     \midrule
%     Exc. B  &  & \best{}     &  & \best{} \\
%             &  &             &  &      \\
%     \bottomrule
% \end{tabular}
% }
% \label{tab:opt_point_metric_append}
% \end{table*}

% \begin{table*}[!htbp]
% \centering
% \caption{
% Probabilistic prediction performance of the mixture models by different training methods (mean and standard errors in two rows).
% The best results are marked in dark grey boxes.
% }
% \resizebox{0.5\textwidth}{!}{
% \begin{tabular}{l|ll|ll}
% \toprule       
%                   & \multicolumn{2}{c|}{NLLm $\downarrow$}                                         & \multicolumn{2}{c}{QLm $\downarrow$} \\
%                   & \multicolumn{2}{c|}{Share}       & \multicolumn{2}{c}{Share}  \\
%     Dataset       & Direct & Phased                  & Direct & Phased          \\
%     \midrule
%     \midrule
%     Site 0  & 4.103 & \best{3.879}          & 0.0582 & \best{0.0463}   \\
%             & 0.133 & 0.011                 & 0.009  & 0.001           \\
%     \midrule
%     Site 1  & 3.772 & \best{3.776}          & 0.0589 & \best{0.0505}    \\
%             & 0.006 & 0.003                 & 0.009  & 0.001            \\
%     \midrule
%     Site 2  & 3.720 & \best{3.679}          & 0.0550 & \best{0.0502}   \\
%             & 0.013 & 0.001                 & 0.002  & 0.001           \\
%     \midrule
%     Site 3  & 4.392 & \best{3.962}          & 0.0669 & \best{0.0471}   \\
%             & 0.029 & 0.001                 & 0.002  & 0.001           \\
%     \midrule
%     Site 4  & 3.948 & \best{3.906}          & 0.0456 & \best{0.0453}  \\
%             & 0.040 & 0.005                 & 0.003  & 0.003          \\
%     \midrule
%     Site 5  & 3.891 & \best{3.866}          & 0.0448 & \best{0.0445}  \\
%             & 0.013 & 0.001                 & 0.001  & 0.001          \\
%     \midrule
%     Site 6  & 3.631 & \best{3.623}          & 0.0466 & \best{0.0470}   \\
%             & 0.002 & 0.001                 & 0.002  & 0.001           \\
%     \midrule
%     Site 7  & 4.137 & \best{3.871}          & 0.0606 & \best{0.0450}  \\
%             & 0.023 & 0.003                 & 0.004  & 0.001          \\
%     \midrule
%     Site 8  & 3.798 & \best{3.765}          & 0.0467 & \best{0.0465}  \\
%             & 0.003 & 0.005                 & 0.001  & 0.001          \\
%     \midrule
%     Site 9  & 4.020 & \best{3.902}          & 0.0518 & \best{0.0461}  \\
%             & 0.025 & 0.004                 & 0.001  & 0.001          \\
%     \midrule
%     Site 10 & 4.096 & \best{3.856}          & 0.0680 & \best{0.0474}  \\
%             & 0.012 & 0.015                 & 0.004  & 0.003          \\
%     \midrule
%     Site 11 & 3.990 & \best{3.938}          & 0.0468 & \best{0.0461}  \\
%             & 0.001 & 0.001                 & 0.005  & 0.001          \\
%     \midrule        
%     \midrule
%     Exc. A  &  & \best{}            &  &     \\
%             &  &                    &  &     \\
%     \midrule
%     Exc. B  &  & \best{}            &  &   \\
%             &  &                    &  &   \\
%     \bottomrule
% \end{tabular}
% }
% \label{tab:opt_prob_metric_append}
% \end{table*}




% \begin{align*}
% \begin{split}
% -\log \mathbb{E}_{\mathbf{h}_{1:S,t}} 
% \left[
% \sum_{s = 1}^{S} \mathbb{P}_{\theta}(z_t = s \,|\, {\mathbf{h}}_{1:S,t}) \, p_{{\omega}_{s}}(y_t \,|\, z_t = s, {\mathbf{h}}_{s,t}) 
% \right] 
% \end{split}
% \end{align*}

% % ------------------------
% \begin{table*}[!htbp]
% \centering
% \caption{
% Point prediction performance of the mixture models by different training methods (mean and standard errors in two rows).
% The best results are marked in $\best{dark}$ grey boxes.
% }
% \resizebox{\textwidth}{!}{
% \begin{tabular}{l|lll|lll|lll|lll}
% \toprule       
%                      & \multicolumn{6}{c|}{RMSE $\downarrow$}                                    & \multicolumn{6}{c}{MAE $\downarrow$} \\
%                      & \multicolumn{3}{c|}{Share}     & \multicolumn{3}{c|}{Resi.}               & \multicolumn{3}{c|}{Share}    & \multicolumn{3}{c}{Resi.} \\
%     Dataset          & Direct & APPRO & Phased        & Direct & APPRO & Phased                  & Direct & APPRO & Phased       & Direct & APPRO & Phased  \\
%     \midrule
%     \midrule
%     Site 0  & 27.173 & 34.686 & \best{19.022}   & 26.430 & 36.574  & \best{18.754}   & 14.905 & 16.324 & \best{10.297}   & 12.247 & 16.047 & \best{10.228} \\
%             & 1.617  & 1.956  & 0.054           & 1.989  & 1.234   & 0.073           & 0.423  & 0.893  & 0.048           & 0.284 & 0.802   & 0.020        \\
%     \midrule
%     Site 1  & 41.549 & 32.430 & \best{18.517}   & 30.937 & 19.558 & \best{17.936}    & 17.876 & 15.978 &\best{9.929}     & 10.741 & 9.923 & \best{9.746} \\
%             & 2.013  & 1.784  & 0.086           & 1.349  & 1.982  & 0.090            & 1.102  & 1.123  & 0.027           & 0.102  & 0.036 & 0.024      \\
%     \midrule
%     Site 2  & 17.279 & 32.996 & \best{17.081}   & 19.148 & 39.817 & \best{17.234}    & 8.832  & 8.878 & \best{8.573}     & 9.416  & 16.040 & \best{8.682} \\
%             & 0.021 & 2.192   & 0.087           & 1.329  & 1.781  & 0.039            & 0.011  & 0.012 & 0.037            & 0.023  & 1.143  & 0.035       \\
%     \midrule
%     Site 3  & 30.509 & 37.579 & \best{21.969}   & 26.717 & 37.374 & \best{21.545}    & 14.241 & 17.189 & \best{11.293}  & 16.448 & 16.374 & \best{11.103} \\
%             & 1.132  & 1.435  & 0.101           & 0.924  & 1.012  & 0.046            & 0.102  & 0.812  & 0.059          & 0.924  & 1.123  & 0.053        \\
%     \midrule
%     Site 4  & 26.592 & 20.057 & \best{19.637}   & 29.713 & 20.127 & \best{19.220}    & 17.908 & 10.539 & \best{10.638}   & 14.273 & 10.547 & \best{10.523} \\
%             & 1.123  & 0.143  & 0.062           & 1.732  & 1.612  & 0.096            & 0.812  & 0.123  & 0.084           & 0.843  & 0.014  & 0.038      \\
%     \midrule
%     Site 5  & 30.233 & 43.414 & \best{20.578}   & 25.777 & 20.803 & \best{20.978}    & 19.843 & 20.973 & \best{10.318}   & 11.486 & 12.383 & \best{10.539} \\
%             & 1.932  & 2.121  & 0.128           & 1.123  & 0.323  & 0.196            & 1.324  & 1.434  & 0.049           & 0.145  & 0.104  & 0.088        \\
%     \midrule
%     Site 6  & 24.004 & 19.032 & \best{17.625}   & 18.265 & 37.983 & \best{18.159}    & 22.274 & 8.883 & \best{8.631}     & 9.670 & 22.225 & \best{8.644} \\
%             & 1.433  & 0.323  & 0.063           & 0.434  & 1.545  & 0.089            & 1.322  & 0.103 & 0.027            & 0.101 & 1.234  & 0.036       \\
%   \midrule
%     Site 7  & 22.654 & 38.536 & \best{19.887}   & 24.950 & 25.239 & \best{18.971}    & 15.551 & 18.485 & \best{10.411}   & 12.399 & 25.239 & \best{10.229} \\
%             & 1.121  & 1.434  & 0.122           & 1.434  & 1.654  & 0.049            & 1.143  & 1.435  & 0.059           & 0.202  & 1.232  & 0.026      \\
%     \midrule
%     Site 8  & 69.885 & 20.674 & \best{19.481}   & 60.947 & 36.942  & \best{19.245}   & 18.619 & 10.041 & \best{10.025}   & 15.619 & 22.212 & \best{10.001} \\
%             & 2.954  & 1.545  & 0.110           & 1.212  & 1.102   & 0.111           & 1.232  & 0.013  & 0.029           & 1.123  & 0.823  & 0.046       \\
%     \midrule
%     Site 9  & 53.530 & 38.026 & \best{18.586}   & 73.151 & 24.337 & \best{18.523}    & 25.555 & 17.151 & \best{10.178}   & 28.715 & 36.383 & \best{10.066} \\
%             & 2.132  & 0.432  & 0.034           & 1.234  & 1.564  & 0.072            & 1.323  & 1.512  & 0.020           & 1.123  & 0.853  & 0.050      \\
%     \midrule
%     Site 10 & 28.426 & 25.836 & \best{19.072}  & 63.488 & 34.132 & \best{17.566}    & 32.878 & 17.597 & \best{9.999}    & 31.264 & 16.051 & \best{9.292} \\
%             & 2.434  & 2.543  & 0.247          & 1.545  & 1.655  & 0.159            & 1.232  & 1.532  & 0.033           & 1.102  & 1.323  & 0.040      \\
%     \midrule
%     Site 11 & 87.015 & 26.234 & \best{23.197}  & 27.971 & 29.101 & \best{22.354}    & 18.667 & 13.432 & \best{11.036}   & 19.378 & 13.101 & \best{10.800} \\
%             & 2.545  & 1.654  & 0.137          & 1.754  & 1.798  & 0.144            & 1.345  & 1.154  & 0.042           & 1.123  & 0.254  & 0.043      \\
%     \midrule        
%     \midrule
%     Exc. A  &  &  & \best{}   &  &  & \best{}       &  &  & \best{}    &  &  & \best{} \\
%             &  &  &           &   &   &             &  &  &            &  &  &      \\
%     \midrule
%     Exc. B  &  &  & \best{}   &  &  & \best{}       &  &  & \best{}    &  &  & \best{} \\
%             &  &  &           &   &   &             &  &  &            &  &  &      \\
%     \bottomrule
% \end{tabular}
% }
% \label{tab:opt_point_metric_append}
% \end{table*}


% \begin{table*}[!htbp]
% \centering
% \caption{
% Probabilistic prediction performance of the mixture models by different training methods (mean and standard errors in two rows).
% The best results are marked in $\best{dark}$ grey boxes.
% }
% \resizebox{\textwidth}{!}{
% \begin{tabular}{l|lll|lll|lll|lll}
% \toprule       
%                   & \multicolumn{6}{c|}{NLLm $\downarrow$}                                         & \multicolumn{6}{c}{QLm $\downarrow$} \\
%                   & \multicolumn{3}{c|}{Share}     & \multicolumn{3}{c|}{Resi.}                    & \multicolumn{3}{c|}{Share}    & \multicolumn{3}{c}{Resi.} \\
%     Dataset       & Direct & APPRO & Phased        & Direct & APPRO & Phased                       & Direct & APPRO & Phased       & Direct & APPRO & Phased   \\
%     \midrule
%     \midrule
%     Site 0  & 4.103 & 4.236 & \best{3.879}   & 4.166 & 4.202 & \best{3.852}          & 0.0582 & 0.0719 & \best{0.0463}    & 0.0592 & 0.0681 & \best{0.0451} \\
%             & 0.133 & 0.143 & 0.011          & 0.051 & 0.031 & 0.002                 & 0.009  & 0.003  & 0.001            & 0.003  & 0.004  & 0.001       \\
%     \midrule
%     Site 1  & 3.772 & 4.167 & \best{3.776}   & 3.789 & 3.784 & \best{3.761}          & 0.0589 & 0.0818 & \best{0.0505}    & 0.0528 & 0.0582 & \best{0.0497} \\
%             & 0.006 & 0.110 & 0.003          & 0.004 & 0.002 & 0.002                 & 0.009  & 0.003  & 0.001            & 0.002  & 0.002  & 0.001      \\
%     \midrule
%     Site 2  & 3.720 & 3.750 & \best{3.679}   & 3.712 & 4.117 & \best{3.680}          & 0.0550 & 0.0524 & \best{0.0502}    & 0.0579 & 0.0846 & \best{0.0494} \\
%             & 0.013 & 0.010 & 0.001          & 0.071 & 0.094 & 0.005                 & 0.002  & 0.004  & 0.001            & 0.003  & 0.006  & 0.001      \\
%     \midrule
%     Site 3  & 4.392 & 4.277 & \best{3.962}   & 4.408 & 4.235 &\best{3.952}           & 0.0669 & 0.0700 & \best{0.0471}    & 0.0924 & 0.0672 & \best{0.0459} \\
%             & 0.029 & 0.001 & 0.001          & 0.021 & 0.073 & 0.007                 & 0.002  & 0.002  & 0.001            & 0.008  & 0.002  & 0.002       \\
%     \midrule
%     Site 4  & 3.948 & 3.925 & \best{3.906}   & 4.122 & 3.925 & \best{3.901}          & 0.0456 & 0.0471 & \best{0.0453}   & 0.0571 & 0.0463 & \best{0.0439} \\
%             & 0.040 & 0.003 & 0.005          & 0.137 & 0.012 & 0.002                 & 0.003  & 0.004  & 0.003           & 0.002  & 0.001  & 0.001        \\
%     \midrule
%     Site 5  & 3.891 & 4.383 & \best{3.866}   & 4.311 & 3.936 & \best{3.875}          & 0.0448 & 0.0864 & \best{0.0445}   & 0.0781 & 0.0429 & \best{0.0441} \\
%             & 0.013 & 0.132 & 0.001          & 0.093 & 0.012 & 0.004                 & 0.001  & 0.010  & 0.001           & 0.004  & 0.005  & 0.001      \\
%     \midrule
%     Site 6  & 3.631 & 3.778 & \best{3.623}   & 3.634 & 4.410 & \best{3.611}          & 0.0466 & 0.0467 & \best{0.0470}   & 0.0468 & 0.107 & \best{0.0463} \\
%             & 0.002 & 0.003 & 0.001          & 0.005 & 0.100 & 0.003                 & 0.002  & 0.004  & 0.001           & 0.002  & 0.003 & 0.001      \\
%     \midrule
%     Site 7  & 4.137 & 4.273 & \best{3.871}   & 4.187 & 4.078 & \best{3.865}          & 0.0606 & 0.0755 & \best{0.0450}   & 0.0609 & 0.0513 & \best{0.0436} \\
%             & 0.023 & 0.012 & 0.003          & 0.112 & 0.064 & 0.002                 & 0.004  & 0.006  & 0.001           & 0.001  & 0.003  & 0.001      \\
%     \midrule
%     Site 8  & 3.798 & 3.847 & \best{3.765}   & 4.330 & 4.429 & \best{3.762}          & 0.0467 & 0.0483 & \best{0.0465}   & 0.0855 & 0.0916 & \best{0.0456} \\
%             & 0.003 & 0.013 & 0.005          & 0.103 & 0.117 & 0.004                 & 0.001  & 0.001  & 0.001           & 0.008  & 0.003  & 0.001   \\
%     \midrule
%     Site 9  & 4.020 & 4.184 & \best{3.902}   & 4.060 & 3.893 & \best{3.870}          & 0.0518 & 0.0741 & \best{0.0461}   & 0.0557 & 0.0472 & \best{0.0440} \\
%             & 0.025 & 0.029 & 0.004          & 0.023 & 0.061 & 0.003                 & 0.001  & 0.003  & 0.001           & 0.003  & 0.001  & 0.002       \\
%     \midrule
%     Site 10 & 4.096 & 4.145 & \best{3.856}   & 4.058 & 4.153 & \best{3.771}          & 0.0680 & 0.0739 & \best{0.0474}   & 0.0625 & 0.0732 & \best{0.0424} \\
%             & 0.012 & 0.011 & 0.015          & 0.043 & 0.078 & 0.003                 & 0.004  & 0.002  & 0.003           & 0.001  & 0.008  & 0.001       \\
%     \midrule
%     Site 11 & 3.990 & 4.116 & \best{3.938}   & 4.071 & 3.967 & \best{3.921}          & 0.0468 & 0.0538 & \best{0.0461}   & 0.0529 & 0.0459 & \best{0.0436} \\
%             & 0.001 & 0.084 & 0.001          & 0.032 & 0.012 & 0.005                 & 0.005  & 0.001  & 0.001           & 0.001  & 0.004  & 0.001      \\
%     \midrule        
%     \midrule
%     Exc. A  &  &  & \best{}   &  &  & \best{}       &  &  & \best{}    &  &  & \best{} \\
%             &  &  &           &   &   &             &  &  &            &  &  &      \\
%     \midrule
%     Exc. B  &  &  & \best{}   &  &  & \best{}       &  &  & \best{}    &  &  & \best{} \\
%             &  &  &           &   &   &             &  &  &            &  &  &      \\
%     \bottomrule
% \end{tabular}
% }
% \label{tab:opt_prob_metric_append}
% \end{table*}







% This would further reinforce the low posterior weights as the training progresses.
% Consequently, we observe the imbalanced learning in Fig.\ref{fig:tr_behaviour}(a). 
% \tian{}

% over the representations is replaced by a single point (i.e. $\widetilde{\mathbf{h}}_{s,t}$),  
% The \textit{Residual} mixture loss can be derived similarly and put in the appendix section. 
% \tian{ $\mathbf{h}_{1:S,t}$, $\mathbf{r}_{s,t}$ }

% & \text{ s.t. } \, \widetilde{\mathbf{h}}_{s,t} = \text{NN}_{\eta_s}(\mathbf{x}_{s, <t}) 
% For most training of deep neural networks, SGD or its variants are used to optimize such loss functions. 
% We assume for a weight vector to have access to a stochastic gradient.
% Minimizing above loss function via SGD style optimization is termed the gradient Expectation Maximization (EM).
% Experimentally, we observe imbalance issues of 

% we can see this effect as learning progress on Dataset A of Sec. 3.1 in Fig. 2.
%  via SGD style optimizations
% imbalanced prediction performance of different data sources, 
% In Fig.~\ref{fig:tr_behaviour}(a), the widely dispersed source-wise prediction errors suggest imbalanced learning status of different data sources, e.g. the high prediction errors could imply under-learned data sources.
% source-wise prediction errors when minimizing Eq.~\ref{eq:loss}.

% Individual source's prediction performance is noticeably improved, compared with the results in Fig.~\ref{fig:tr_behaviour}(a).
% In Fig.~\ref{fig:tr_behaviour}(b), some sources are revealed to bear decent predictive power, while undiscovered during the training in Fig.~\ref{fig:tr_behaviour}(a).

% It shows that source-wise errors are widely dispersed, and the high error curves imply the potential
% likely to be under-learned, prediction modules of the corresponding data sources.
% hardly learned, considerable spread, gap
% it is unclear under-learned or the predictive power, if it is the latter case, 
% exhibit different convergence
% during the phased training under the same setup as Fig.~\ref{fig:tr_behaviour}(a).

% hinder, Because of this imbalanced and unstable behaviour, the weight module would hardly learn accurate combination of individual density functions, thereby impairing the mixture's prediction performance.

% Considering distinct learning difficulties of data sources, the corresponding prediction and representation modules are in different learning status in the training.
% while other data sources would improperly receive high posterior weights, 
% Meanwhile, other data sources would improperly receive higher posterior weights, 

% and this update bias would persist in the training.

% when a data souurce has prediction density  weights

% For some under-learned data sources, the low prediction density and premature weights of these sources could lower down the posterior weights i.e. Eq.~\ref{eq:post_weight}, which in turn further slow down the update of these modules i.e. Eq.~\ref{eq:update_content}.

% \tian{practically}
% This bias would persist during the training.
% could be over-fitted 
% Overfitting others
% Consequently, some source's predictive power  and barely 
%  e.g. $\mathbb{P}_{\theta}(z_t = s | \cdot)$ and $p_{{\omega}_{s}}(y_t | \cdot)$,  $\pi_{s,t}$
% Consequently, each source's parameters would be biasedly updated because of the $\pi_{s,t}$ weighted derivatives, as is shown in Eq.~\ref{eq:update}.
% some data source's predictive density could quickly learn decent density function, while some could take longer time.
% \tian{uniform prior,  “die” during training, since by sharing pa-rameters even unpopular experts receive some gradients.}
% faithfully/

% impartial phase and {collective phase},.
% In the first \textit{impartial phase}, the sharing representation and source-wise prediction modules are learned to unbiasedly capture the predictive power of individual data sources.
% In the subsequent \textit{collective phase}, the weigh module (with the residual representation in \textit{Residual} mixture) is then activated to learn collective predictions with adaptation.

% related parameters in an equal-weighted manner. 
% thereby merely updating the predictive
% nspired by Lemma~\ref{theo:bound_loss},
% density and sharing representation related parameters in an equal-weighted manner. 
% The corresponding stochastic update is becoming:\tian{only predictive power, no matter weight}



% In Eq.\ref{eq:share}, the three modules will be learned in two phases of proposed phased learning in Sec.~\ref{sec:tr}.
% The sharing representation and prediction modules are learned in the first phase for capturing predictive power of individual data sources, followed by
% the weight module to learn adaptive combinations in the second phase.

% and learned in the second phase
% as $\mathbf{h}_{1:S,t}$ is learned in the first phase for capturing the predictive power of data, 
% $\mathbf{r}_{1:S,t}$ will be incorporated into the weight module and learned in the second phase to provide supplementary information for the weight module.
% \tian{thus independent relation, decomposed as}


% is becoming high in Fig.\ref{fig:output_example}(b).
% In Fig.\ref{fig:output_example}(c), the mixture uncertainty is driven up by the prediction dispersion of distinct sources. 

% in the work of stochastic neural networks and ensemble methods where 
% In many existing works (e.g., Bayesian or stochastic neural networks, ensemble methods, etc.), the uncertainty quantification methods usually utilize equal-weighted samples of model parameters or latent states~\cite{gal2016dropout, lakshminarayanan2017simple, qiu2021history}.
% In future work, it is also feasible to incorporate the posterior samples of model parameters into our mixture structures.

% , and together with the mixture uncertainty it is driving up the total uncertainty to reflect the potential unreliability of the predictions in this period.

% Overall the total uncertainty is driven up to reflect the potential unreliability of the predictions in period \circled{2}.
% \tian{reveal data source provide different prediction regions}

% and lead to the high mixture uncertainty as is shown . 
% \tian{weight server, different from existing works}
% to reflect the reliability of predictions

% the predictive aleatoric uncertainty is rising in Fig.~\ref{fig:output_example}(b).
% Furthermore, as  when the target 
% The predictions mainly distribute on the high value range, and it is likely that only few data sources are able to provide predictions on that level, and therefore the mixture uncertainty is high.
% The resulting high overall uncertainty raises the awareness of potentially increasing prediction errors.
% model uncertainty into mixture models by
% prediction has low 
% These predictions are mostly in the low value range, and the mixture uncertainty is relatively low in \circled{1}.
% thereby fluctuating with small magnitudes, as is shown in the top panel. 
% This will motivate the proposal of the phased training method in the next subsection.
% \tian{using one random sample, we stick to a single datum for cleaner presentation}


% The sharing and prediction module parameters are updated as Eq.\ref{eq:update_content}.
% It amounts to fine-tuning the sharing representation and prediction module by taking into account the relevance disparity of data sources which is reflected in the posterior weights in Eq.\ref{eq:update_content}.
% The posterior weight in Eq.\ref{eq:update_content} reflects different data sources' relevance to the target, and thus in this \textit{collective phase}, 

% taking into account the beliefs of data source's relevance to the target different relevance beliefs.

% In the \textit{Residual} mixture, the residual representations are only learned in the \textit{collective phase}.
% The stochastic update to the residual parameters $\{\tau_s\}_{s=1}^S$ is only through the weight module
% adaptation.
% Owing to the sharing representations and prediction modules reasonably learned in the \textit{impartial phase}, the mixture can learn to make accurate collective predictions in this phase.
% \tian{residual adjust}
% , unlike the sharing representation updated through both the prediction and weight modules as shown in Eq.\ref{eq:update_content}.
% \tian{}


% the abundant information and 
% complex patterns in 
% , and these multi-source data further motivate the need for powerful modelling methods.
%  mixture models on
% For capturing various and time-varying relevance of multi-source data to the target, 
% Specifically, we focus on the forecasting mixture model, which 
% The probabilistic mixture model is aimed to capture various and time-varying relevance of input data to the target variable, and particularly suited for multi-source data.
% Methodologically, we explore the mixture structure from the perspective of data representations and weight mechanisms, thereby leading to two specific structures, i.e. \textit{Sharing} and \textit{Residual} mixtures.
% \tian{
% On the inference side, we present the favorable properties of the adaptive point prediction and the associated predictive uncertainty.
% % contribution weights.
% On the learning side, after analyzing the imbalance and unstable training behaviors of the forecasting mixtures, 
% we propose the phased training method, so as to stably learn data source's predictive power as well as the collective prediction
% providing theoretical insights.


% \tian{This allows for any choice of appropriate integration method}

% \tian{A set of novel approaches for estimating epistemic uncertainty in deep neural
% networks with a single forward pass has}

% A possible formulation can be expressed as: 
% $p( \mathbf{h}_{1:S,t}, \mathbf{h}_{0,t} \,|\, \mathbf{x}_{1:S,<t} ) = \prod_{s=1}^S p( \mathbf{h}_{s,t} \,|\, \mathbf{h}_{0,t}, \mathbf{x}_{s,<t} ) \cdot p( \mathbf{h}_{0,t} \,|\, \mathbf{x}_{1:S,<t} )$, where $\mathbf{h}_{0,t}$ denotes the global representation.

% \begin{align}
% \begin{split}
% & p( \, \mathbf{r}_{1:S, t} \,|\, \mathbf{x}_{1:S,<t} ) = \prod_{s=1}^S \delta(\mathbf{r}_{s,t} - \widetilde{\mathbf{r}}_{s,t}) \\
% & \text{s.t.} \, \widetilde{\mathbf{r}}_{s,t} = \text{NN}_{\eta_s}(\mathbf{x}_{s, <t}), \forall s = 1, \cdots, S
% \end{split}
% \end{align}
% \tian{}
% , given the covariates of the next time point ct, via the updated hidden state ht1:
% (Autoregressive Denoising Diffusion Models for Multivariate Probabilistic Time Series Forecasting)
% \underline{Future work}, common factors
% discuss: common factors, either added into individual representation, or another new component model
% In this section, we first present some favorable properties of the inference, and then the learning process.
% \textbf{[key elements]: adaptive point and quantile prediction, uncertainty quantification, }
% Based on the data dependent weights capturing the varying contribution of each data source, it is expressed as:


% for different domains of $y_t$, we focus on two distributions, namely, normal distribution for $y_t \in \mathbb{R}$, and log-normal distribution for $y_t \in \mathbb{R}^{+}$~\cite{cohen1980estimation, mackay2003information}, while other distributions are potentially allowed. 


% [key elements]: disentangled representations, temperature scaling in the gate function,
% In this part, we first present the general framework of the forecasting mixture, and then elaborate on two specific structures. 
% from the roles of multi-source data representations and the weighting mechanism



% , since it will be jointly learned. 
% i.e. $f_{\theta_s}( \cdot ): \mathbb{R}^{d_s} \rightarrow \mathbb{R}$, where $d_s$ is the dimensionality of $\mathbf{h}_{s,t}$ and 



% but in this work, we focus on investigating these two fundamental ones which could inspire future work.
% \tian{from a learning perspective, we argue that the fixed topology may restrict the model capacity and thus potentially hinder the performance}, hinder the overall performance of the mixture
% The sharing representation learned in the first phase mainly serves the prediction module.
% In particular, we incorporate $\mathbf{r}_{1:S,t}$ into the weight module.
% \tian{$\mathbf{r}_{1:S,t}$ will be learned in the second phase of 
%  as $\mathbf{h}_{1:S,t}$ and is expected to capturing supplementary information for the weight module.}




%  modern datasets are frequently assembled by merging data from multiple sources without explicit source label

% Assume the \textit{Sharing} and \textit{Residual} mixture loss are $L$-smooth.
% For all stochastic derivatives $\mathbf{g} \in \{\mathbf{g}_{\omega_{s}}, \mathbf{g}_{\eta_{s}}, \mathbf{d}_{\eta_{s}}\}_{s=1}^S \cup \mathbf{g}_{\theta}$, it has the bounded norm $\mathbb{E}\lVert \mathbf{g} \rVert^2 \leq G^2$ and the bounded variance $\mathbb{E} \lVert \mathbf{g} - \mathbb{E}[\mathbf{g}] \rVert^2 \leq \zeta^2$.
% For the learning iteration step $i = 0, \cdots, I$, the value of trainable parameters at $i$ is denoted by $\Theta_i$, of which the weight module parameter $\theta$ is constant, since it is not updated in the impartial phase. 

% Then, in the \textit{impartial phase}, as the parameters $\{\eta_s, \omega_s\}_{s=1}^S$ are updated through minimizing $\overline{\mathcal{L}}\big( \{\eta_s, \omega_s\}_{s=1}^S \big)$, in expectation the overall loss function $\mathcal{L}\left( \Theta \right)$ converges towards (a neighborhood of) a stationary point by the following:
% \begin{align}
% \begin{split}
% & \frac{1}{I+1} \sum_{i=0}^I \mathbb{E}[ \norm{\nabla \mathcal{L}(\Theta_i)}^2 ]  
% \leq \\
% & \frac{2S\mathbb{E}[\mathcal{L}\left( \Theta_{I} \right)] - \mathbb{E}[\mathcal{L}\left( \Theta_{0} \right)]}{\mu (I+1)} 
%  + 2 (S \zeta^2 + S G^2 + \mu L G^2) 
% \end{split}
% \end{align}

% \tian{We complement the proposed CO framework with a powerful empirical Bayes prior}

% We introduce the basic data representation of multi-source data, namely the sharing representation $\mathbf{h}_{1:S,t}$, a set of the representation vectors $\{ \mathbf{h}_{s,t} \}_{s=1}^{S}$ learned from $\mathbf{x}_{1:S,<t}$.

% By pooling the predictive representations of data sources and re-arranging the terms in Eq.~(\ref{eq:overall_model}),
% \tian{why weight,  and useful for the weigh module}

% In the following, we will show this residual weight module implicitly amounts to being equipped with a learnable temperature scaling mechanism.

% Meanwhile, in our proposed phased training method in Sec.~\ref{sec:tr}, sharing and residual representations are learned in different phases

% is intended for providing supplementary representations, given that

% Concretely, by introducing the residual representations denoted by $\mathbf{r}_{1:S,t}$, the weight module makes use of two complementary sets of representations, thereby leading to the factorization as follows:

% enables to capture residual useful information in data for the weight module.

% provide supplementary information for the weight module.

% We will show this residual weight module implicitly amounts to being equipped with a learnable temperature scaling mechanism in the following.

% additional capacity
% for providing supplementary representations

% Besides the sharing representations, there could be residual useful information left in data~\cite{?} and therefore, we introduce the residual representations denoted by $\mathbf{r}_{1:S,t}$.



% Given the learned parameters, several predictive quantities can be derived from the multi-modal distribution of the target~\cite{mackay2003information, yuksel2012twenty}.
% \tian{multi step ahead i.e. from $t-1$, $t-2$ until the look-back horizon}.
% We assume $\{\mathbf{x}_{s,<t}\}_{s=1}^{S}$ could have different dimensions of variables/features and window lengths. 
% $p(\, y_t \,|\, \{\mathbf{x}_{s,<t}\}_{s=1}^{S})$.
% Then, let $\mathbf{x}_{1:S,<t}$ be the data from $S$ sources $\{\mathbf{x}_{s,<t}\}_{s=1}^{S}$

% We assume that there is access to a historical dataset
% However, we argue that learning from a single time series while useful in cases where indeed only one time-series is available 
% may not be optimal in settings where datasets contain multiple time-series, the shared patterns of which could potentially be exploited (Figure 1, right)
% A forecasting model capable of capturing the time-varying relevance of the multi-source data to the target variable
% We address the task of discrete-time multivariate time-series prediction, with the goal of forecasting multiple time-steps ahead. 
% The model developed below is flexible to consume multi-source data of arbitrary number of sources and dimensionalities of individual source data.
% We assume that there is access to a historical dataset for training, but after training the model must perform prediction based on a limited window of historical data.
% For simplicity, we will use one data sample of the target $y_t$ to present the proposed model.
% In reality, the training, validation, and testing data contain the samples collected in a time period.
% More quantitatively, the generative process of the target variable $y_t$ conditional on multi-source data $\{\mathbf{x}_{1,t}, \cdots, \mathbf{x}_{S,t}\}$ is formulated as the following probabilistic mixture process:
% \begin{align}
% \label{eq:joint}
% p(\, y_t \,|\, \{\mathbf{x}_{s,<t}\}_{s=1}^{S} )
% \end{align}
% is a probability distribution parameterized by. 
% In our experiments, G is a normal distribution with mean and constant diagonal varian (Stochastic Latent Residual Video Prediction)
% As d is fixed, we will abbreviate dk=1 x k by k x k throughout.
% Formally, given a source sentence x and reference translation y, a mixture model introduces a multinomial latent variable % z ∈ {1, · · · , K}, 
% and decomposes the marginal likelihood as:

% a predictive density function conditional on each data-source-wise prediction models.
% density function.
% 's contribution to $p(y_t \,|\, \mathbf{x}_{1:S,<t})$.

% , which will be used to decompose the target density function $p(y_t \,|\, \{\mathbf{x}_{s,<t}\}_{s=1}^{S} )$.
% \tian{role}In neural network based forecasting, a continuous representation is normally learned from the input data and then used as the predictive feature to subsequent models.

% \tian{in our case, z is in 1...S }
% Then, let $z_t$ be a discrete random variable defined on the data source index set i.e. $z_t \in \{1, \cdots, S\}$.
% Then, each data source has a corresponding prediction model using the predictive representation and the probability function of $z_t$ serves as the time-varying weight of each data source's contribution to $p(y_t \,|\, \mathbf{x}_{1:S,<t})$.

% Specifically, the factorization of the joint distribution is as:
% \begin{align}\label{eq:overall_model}
% % & p(\, y_t \,|\, \{\mathbf{x}_{s,<t}\}_{s=1}^{S} ) = 
% \int \sum_{s=1}^S 
% \underbrace{\mathbb{P} \Big(z_t=s \Big| \cdot \Big)}_{\text{weight module}} 
% \underbrace{p \Big( y_t \Big| z_t=s, \mathbf{h}_{s,t} \Big)}_{\text{prediction module}} 
% \underbrace{p \Big(\mathbf{h}_{s,t} \Big| \mathbf{x}_{s,<t} \Big)}_{\text{representation module}}
% \text{d}\mathbf{h}_{1:S,t}
% \end{align}
% \begin{align}\label{eq:overall_model}
% \int 
% \underbrace{p(\mathbf{h}_{1:S,t} | \mathbf{x}_{1:S,<t})}_{\text{representation module}}
% \sum_{s=1}^S 
% \underbrace{\mathbb{P}(z_t=s | \cdot )}_{\text{weight module}} \,
% \underbrace{p(y_t | z_t=s, \mathbf{h}_{s,t})}_{\text{prediction module}} 
% % \underbrace{p(\mathbf{h}_{s,t} | \mathbf{x}_{s,<t})}_{\text{representation module}}\text{d}
% \mathbf{h}_{1:S,t}
% \end{align}
% $z_t$ is a multinomial random variable and 
% , where the probability function of $z_t$, i.e. $\mathbb{P}(z_t=s|\cdot)$, serves as the time-varying weight of each data source's contribution to the overall density function.
% Each data source has the corresponding prediction model using the predictive hidden representation.
% satisfying $\sum_{s=1}^S \mathbb{P}(z_t=s|\cdot) = 1$, 
% In Eq.~(\ref{eq:overall_model}), we leave a degree of freedom on the weight module, because we will present two specific designs, i.e. \textit{Sharing} and \textit{Residual} mixtures.

% For instance, Fig.~\ref{fig:tr_behaviour}(b) shows the source-wise prediction errors during the phased training under the same setup as Fig.~\ref{fig:tr_behaviour}(a).
% Individual source's prediction performance is noticeably improved, compared with the results in Fig.~\ref{fig:tr_behaviour}(a).
% In Fig.~\ref{fig:tr_behaviour}(b), some sources are revealed to bear decent predictive power, while undiscovered during the training in Fig.~\ref{fig:tr_behaviour}(a).
% Furthermore, the overall prediction performance of mixture models is enhanced, as is demonstrated in Sec.~\ref{sec:exp}.
% despite the impartial learning phase is focused on the subset of $\Theta$,


% , i.e., $\Theta_i = \big\{ \{\eta_{s,i}, \omega_{s,i} \}_{s=1}^S, \theta_{0} \big\}$.
% \textbf{? partial gradient clipping}, the number of phase epoch fix or as hyper parameter, prediction interval
% The rightmost term in (2) measures the average quality of the pruning. 
% However, unless  or , the error term never completely vanishes, meaning that the method converges only to a neighborhood of the optimal solution (this not only holds for the pruned model, but also for 3Our variable wt corresponds to x˜t in the notation of Karimireddy et al. (2019). 
% Their error-fixed SGD algorithm evaluates gradients at perturbed iterates , which correspond precisely to  in our notation. This shows the connection of these two methods.
% the jointly maintained dense model, as we will show in the appendix). 
% This behavior is expected, as the global optimal model w? might be dense and cannot be approximated well by a sparse model.


% suggest imbalanced predictive power.
% predictive power is under-learned, thereby leading to high errors.

% Consequently, the weight module  
% This would also pose challenges for the weight module to learn proper combination 
% are dispersed in a wide range and the high error curves suggest some source's predictive power are density functions are under-learned  insufficient predictive power learned from the corresponding sources during the training.

% \tian{Second, the wide error bars suggest unstable training processes. 
% Consequentially, the weight module could hardly learn reliable weights and the overall prediction performance of mixtures would be harmed as well.}
% \tian{overconfident, under learned, under trained}
% \tian{even if some data sources are redundant, multi-choice learning}
% \tian{Both extreme cases can greatly degrade the predictive performance, as shown in the experiments}

% untrained source are not mitigated over the training phase, 
% between the true value and mean by each predictive density function, during the training with the loss function, 
% third, imbalance, high variation, 
% overall prediction performance harmed, 
% misleading interpretation, 
% \tian{gradient EM} In the iterative process of stochastic gradient decent, at every training step $i$, a mini-batch of training examples is sampled to calculate a stochastic gradient for updating model parameters.
% $t$ represent the sample instance. 

% residual model, representation only through gate
% regularization effect

% \tian{Neutral phase, impartial phase, collective}

% The idea is to have two phases to train different modules of the mixture. 

% the multi-modal density of the target.

% the individual modalities are learnt faithfull
% This ensures that all parameters are optimised individually to their best possible extent instead
% of down-weighting less informative so
% Global phase: $ \mathcal{L}\left( \Theta \right) $, the component specific parameters, 
% Then, when the learning switch to the global phase,  all parameters are jointly updated to minimize the overall loss function,
% jacobia matrix to explain gradient update,
% notably,
% we first present a theoretical observation which motivates 
% based on Lemma~\ref{theo:bound_loss}, update the sharing representation and predictive density function related parameters
% Compared with Eq.~\ref{eq:update}, data source specific parameters are equally importantly updated and 


% phase 1, bound, distance to original update, variance

% $\overline{\mathcal{L}}\big( \{\eta_s, \omega_s\}_{s=1}^S \big) = - \sum_{s = 1}^{S} \frac{1}{S} \log  p_{\omega_s}(y_t \,|\, z_t = s, \widetilde{\mathbf{h}}_{s,t} ), \text{  }$
% i.e. $\Theta = \left\{ \{\eta_s, \omega_s\}_{s=1}^S, \theta \right\}$ or $\Theta = \left\{ \{\eta_s, \omega_s\}_{s=1}^S, \theta, \{\tau_s\}_{s=1}^S \right\}$.
% The right hand side of Eq.~\ref{eq:bound} depends on the component specific parameter.
% The phased learning method is proposed based on the following idea.
% the individual modalities are learnt faithfull
% This ensures that all parameters are optimised individually to their best possible extent instead
% of down-weighting less informative so
% the parameter set $\{\eta_s, \omega_s\}_{s=1}^S$ will be updated through the gradient of the first term on the right hand side.
% Then, the bound constantly holds, regardless of updating the rest of parameters of the original loss function. 
% requiring artificial subsampling of the observations to ensure that


% and severs to weight the data source specific gradient.
% The SGD training setup is as follows: loss function, SGD setup
% $\Theta = \left\{ \{\eta_s, \omega_s\}_{s=1}^S, \theta \right\}$ or $\Theta = \left\{ \{\eta_s, \omega_s\}_{s=1}^S, \theta, \{\tau_s\}_{s=1}^S \right\}$
% yet still incompletely understood,
% We consider the training of a non-convex loss function f : Rd → R. 

% Gradient Contributions
% \textbf{ELBO training}, strict lower bound

% hardly reflects the predictive power of each data source

% $\pi_{s,t}$ is derived from the prior and prediction density of each data source given the current parameter values (e.g. $\Theta_i$)

% Then, $\pi_{s,t}$ would biasedly weight the gradient update for each data source. Then, in the following update, the $\pi_{s,t}$ of inforce the .

% , and hardly reflect the predictive power of each data source.

% In Eq.~\ref{eq:post_weight}, $\pi_{s,t}$ is the posterior weight given the current value of the parameters (e.g. $\Theta_i$) and severs to weight the data source specific gradient.

% premature weighting, biased weight, lead to relation under-learned, the overall performance would be harmed. 

% premature weight, representation is not fully learned, weight individual samples in, one update, 
% hardly reflect the predictive power of each data source, $\pi_{s, t}$ is the posterior weight.

% the weights guide the learning of individual source's models
% taking into account the predictive power of each data source and the prior weight.
% It is derived from the current parameter concerning the prediction, representation and weight modules.

% $\mathcal{L}\left(\{\eta_s, \omega_s\}_{s=1}^S, \theta \right)$
% $\mathcal{L}\left(\{\eta_s, \omega_s\}_{s=1}^S, \theta, \{\tau_s\}_{s=1}^S \right)$

% The issue is that in the training phase, inherent characteristics, data source data present distinctly difficulty learn, depending on the relevance strength,


% \begin{equation}
% - \sum_{s = 1}^{S} \nabla \left[ \mathbb{P}_{\theta}(z_t = s \,|\, \cdot) \, \log p_{{\omega}_{s}}(y_t \,|\, z_t = s, \widetilde{\mathbf{h}}_{s,t}) \right]
% \end{equation}
% $\text{p}_{s, t} = \mathbb{P}_{\theta}(z_t = s \,|\, \cdot)$

% $\text{Global phase: } \pi_{s,t}\mathbf{g}_{\omega_{s}} \,\text{and} \text{ }\, \pi_{s,t} \mathbf{g}_{\eta_{s}} + \mathbf{d}_{\eta_{s}}$

% correct the prior 

% Then the parameters are adjusted according to the descent direction of the expected loss on the mini-batch.
% $\Theta_i = \left\{ \{\eta_{s,i}, \omega_{s,i}\}_{s=1}^S, \theta_i \right\}$ or $\Theta_{i} = \left\{ \{\eta_{s,i}, \omega_{s,i}\}_{s=1}^S, \theta_i, \{\tau_{s,i}\}_{s=1}^S \right\}$

% Let’s consider vanilla SGD:
% A stochastic gradient optimizer refers to an iterative algorithm that repeatedly updates model parameters with a uniformly sampled minibatch of training examples. 
% Concretely, this stochastic gradient with mini-batch size M is computed as follows:
% For any iterative stochastic gradient optimizer 

% g(w) ∈ Rd such that E[g(w)] = ∇f(w). 
% This corresponds to the standard machine learning setting with g(w) representing a (mini-batch) gradient of one (or several) components of the loss function. 
% Stochastic Gradient Descent (SGD) computes a sequence of iterates by the update rule
% $\nabla \mathcal{L} \big( \{\eta_{s}, \omega_{s}\}_{s=1}^S, \theta \,;\, \mathcal{D} \big) = \mathbb{E}_t[\mathbf{g} ]$

% $\mathbf{g} = \nabla \mathcal{L} \big( \{\eta_{s,i}, \omega_{s,i}\}_{s=1}^S, \theta_i \,;\, y_t, \{\mathbf{x}_{s,<t}\}_{s=1}^{S} \big)$
% Without the loss of generality, in the proof we treat the mini-batch M = 1.

% the mini-batches. 
% At each iteration, we assume access to an unbiased stochastic gradient 
% % E[g(x)] = ∇f(x, ξ) 
% corresponding to the paramet
% The loss function that corresponds to the i-th data sample is denoted by 

% \textbf{two ways of training}
% immature weighting, distort, 
% intertwined effect,
% assume the prior are roughly equal, the weights guide the learning of individual source's models,

% poor convergence, fail to, incompletely make fully use of individual source predictive power, overall performance on different metrics,
% we develop some intuition for this phenomenon.
% misleadingly weight,

% \begin{align}
% -\sum_{s = 1}^{S} \pi_{s, t} \nabla \log\big[ p_{{\omega}_{s}}(y_t | z_t = s, \widetilde{\mathbf{h}}_{s,t}) \, \mathbb{P}_{\theta}(z_t = s | \cdot) \big] 
% \end{align}

% In stochastic gradient decent style training, given a random training sample, the vectorized derivative of the component model w.r.t. the prediction and representation parameters are defined as:
% \begin{align}
% & \mathbf{g}_{\omega_{s}} \triangleq -\frac{\partial \log p_{\mathbf{\omega}_{s}}(y_t \,|\, z_t = s, \widetilde{\mathbf{h}}_{s,t})}{\partial \omega_{s}} \Big|_{\Theta_i} \\
% &\mathbf{g}_{\eta_{s}} \triangleq -\frac{\partial \log p_{\omega_{s}}(y_t \,|\, z_t = s, \widetilde{\mathbf{h}}_{s,t})}{\partial \widetilde{\mathbf{h}}_{s,t}} \nabla\widetilde{\mathbf{h}}_{s,t} \Big|_{\Theta_i} \\
% & \mathbf{d}_{\eta_{s}} \triangleq \sum_{k=1}^{S} \pi_{k,t} \frac{\partial \log\mathbb{P}_{\theta}(z_{t} = k | \cdot)}{\partial \widetilde{\mathbf{h}}_{s,t}} \nabla\widetilde{\mathbf{h}}_{s,t} \Big|_{\Theta_i}
% \end{align}

% given the partial derivative $\mathbf{g}_{\omega_{s}} \triangleq -\frac{\partial \log p_{\mathbf{\omega}_{s}}(y_t \,|\, z_t = s, \widetilde{\mathbf{h}}_{s,t})}{\partial \omega_{s}} \Big|_{\Theta_i}$
% $\mathbf{g}_{\eta_{s}} \triangleq -\frac{\partial \log p_{\omega_{s}}(y_t \,|\, z_t = s, \widetilde{\mathbf{h}}_{s,t})}{\partial \widetilde{\mathbf{h}}_{s,t}} \nabla\widetilde{\mathbf{h}}_{s,t} \Big|_{\Theta_i}$
% $\mathbf{d}_{\eta_{s}} \triangleq \sum_{k=1}^{S} \pi_{k,t} \frac{\partial \log\mathbb{P}_{\theta}(z_{t} = k | \cdot)}{\partial \widetilde{\mathbf{h}}_{s,t}} \nabla\widetilde{\mathbf{h}}_{s,t} \Big|_{\Theta_i}$
% where $\pi_{s,t}$ is defined as in Eq.~\ref{eq:weight} and $\mathbf{d}_{\eta_{s}} \triangleq \sum_{k=1}^{S} \pi_{k,t} \frac{\partial \log\mathbb{P}_{\theta}(z_{t} = k | \cdot)}{\partial \widetilde{\mathbf{h}}_{s,t}} \nabla\widetilde{\mathbf{h}}_{s,t}$

% \begin{lemma}\label{lemma:bound}
% In the component and global phase, the stochastic gradient used to update the individual data source's forecasting and representation parameters are respectively formulated as:
% \begin{align*}
% & \text{Component phase: } \frac{1}{S}\mathbf{g}_{\omega_{s}} \,\text{and} \text{ }\, \frac{1}{S}\mathbf{g}_{\eta_{s}}  \\ 
% & \text{Global phase: } \pi_{s,t}\mathbf{g}_{\omega_{s}} \,\text{and} \text{ }\, \pi_{s,t} \mathbf{g}_{\eta_{s}} + \mathbf{d}_{\eta_{s}}
% \end{align*}
% where $\pi_{s,t}$ is defined as in Eq.~\ref{eq:weight} and $\mathbf{d}_{\eta_{s}} \triangleq \sum_{k=1}^{S} \pi_{k,t} \frac{\partial \log\mathbb{P}_{\theta}(z_{t} = k | \cdot)}{\partial \widetilde{\mathbf{h}}_{s,t}} \nabla\widetilde{\mathbf{h}}_{s,t}$
% \end{lemma}

% $\text{Global phase: } \pi_{s,t}\mathbf{g}_{\omega_{s}} \,\text{and} \text{ }\, \pi_{s,t} \mathbf{g}_{\eta_{s}} + \mathbf{d}_{\eta_{s}}$
% \begin{align}\label{eq:weight}
% \begin{split}
% \pi_{s, t} & \triangleq p(z_t = s \,|\, y_t, \mathbf{x}_{1:S,<t} ; \Theta_i) \\
% & = \frac{p_{{\omega}_{s}}(y_t \,|\, z_t = s, \widetilde{\mathbf{h}}_{s,t}) \, \mathbb{P}_{\theta}(z_t = s \,|\, \cdot)}{\sum_{k = 1}^{S} p_{{\omega}_{k}}(y_t \,|\, z_t = k, \widetilde{\mathbf{h}}_{k,t}) \, \mathbb{P}_{\theta}(z_t = k \,|\, \cdot)}  
% \end{split}
% \end{align}


% \begin{equation}
% \frac{1}{S} \mathbf{g}_{\omega_{s}} \text{ and } \pi_{s,t}\mathbf{g}_{\omega_{s}} 
% \end{equation}

% \begin{minipage}{0.47\textwidth}
% \begin{align}
% \text{Component phase } \frac{1}{S} \mathbf{g}_{\omega_{s}},    \pi_{s,t}\mathbf{g}_{\omega_{s}}
% \end{align}
% % \equationset{Component phase}\label{eqset:1}
% \end{minipage}%
% %\hfill\vline
% \hfill
% \begin{minipage}{0.47\textwidth}
% \begin{align}
% \text{Global phase }  \frac{1}{S} \mathbf{g}_{\eta_{s}} , \pi_{s,t} \mathbf{g}_{\eta_{s}} + \mathbf{d}_{\eta_{s}}
% \end{align}
% % \equationset{Global phase}\label{eqset:2}
% \end{minipage}


% \begin{lemma}\label{lemma:dist}
% Let $\begin{bmatrix} \mathbf{g}_{\eta_{s,i}} \\ \vdots \\ \mathbf{g}_{\omega_{s,i}} \end{bmatrix} $ be the derivative vector composed of the stochastic derivative w.r.t. the prediction and representation parameters of each data source, where $s \in \{1, \cdots, S\}$.
% $\begin{bmatrix} \pi_{s,i} \mathbf{g}_{\eta_{s,i}} \\ \vdots \\ \pi_{s,i} \mathbf{g}_{\omega_{s,i}} \end{bmatrix}$ represents the corresponding weighted one.
% There exists the following inequality about the distance between the expected gradient vector and the weighted one:
% \begin{align}
% \left\lVert 
% \mathbb{E} \begin{bmatrix} \mathbf{g}_{\eta_{s,i}} \\ \vdots \\ \mathbf{g}_{\omega_{s,i}} \end{bmatrix} 
% - 
% \mathbb{E} \begin{bmatrix} \pi_{s,i} \mathbf{g}_{\eta_{s,i}} \\ \vdots \\ \pi_{s,i} \mathbf{g}_{\omega_{s,i}} \end{bmatrix}
% \right\rVert^2
% \leq 
% \mathbb{E} \left\lVert \begin{bmatrix} \mathbf{g}_{\eta_{s,i}} \\ \vdots \\ \mathbf{g}_{\omega_{s,i}} \end{bmatrix} \right\rVert^2
% \end{align}
% \end{lemma}

% \begin{proof}

% \begin{align}
% \left\lVert 
% \mathbb{E} \begin{bmatrix} \mathbf{g}_{\eta_{s,i}} \\ \vdots \\ \mathbf{g}_{\omega_{s,i}} \end{bmatrix}
% - \mathbb{E} \begin{bmatrix} \pi_{s,i} \mathbf{g}_{\eta_{s,i}} \\ \vdots \\ \pi_{s,i} \mathbf{g}_{\omega_{s,i}} \end{bmatrix}
% \right\rVert^2
% & = 
% \left\lVert 
% \mathbb{E}\begin{bmatrix} (1-\pi_{s,i}) \mathbf{g}_{\eta_{s,i}} \\ \vdots \\ (1-\pi_{s,i}) \mathbf{g}_{\omega_{s,i}} \end{bmatrix}
% \right\rVert^2 \\
% & \leq 
% \mathbb{E}\left\lVert \begin{bmatrix} (1-\pi_{s,i}) \mathbf{g}_{\eta_{s,i}} \\ \vdots \\ (1-\pi_{s,i}) \mathbf{g}_{\omega_{s,i}} \end{bmatrix} \right\rVert^2 \\
% & =
% \mathbb{E}\left[ \sum_{s=1}^S (1-\pi_{s,i})^2 (\norm{\mathbf{g}_{\eta_{s,i}}}^2 + \norm{\mathbf{g}_{\omega_{s,i}}}^2) \right] \\
% & \leq
% \mathbb{E}\left[ \sum_{s=1}^S (\norm{\mathbf{g}_{\eta_{s,i}}}^2 + \norm{\mathbf{g}_{\omega_{s,i}}}^2) \right] \\
% & =
% \mathbb{E} \left\lVert \begin{bmatrix} \mathbf{g}_{\eta_{s,i}} \\ \vdots \\ \mathbf{g}_{\omega_{s,i}} \end{bmatrix} \right\rVert^2
% % = \frac{1}{S} \mathbb{E}[ \norm{\mathring{\mathbf{g}}_i}^2 ]
% \end{align}

% \end{proof}


% share version of the model

% \begin{proof}

% it is

% $\mathbf{g}_{\omega_{s,i}} = -\frac{\partial \log p_{\mathbf{\omega}_{s,i}}(y \,|\, z = s, \widetilde{\mathbf{h}}_{s,i})}{\partial \omega_{s,i}} $

% $\mathbf{g}_{\eta_{s,i}} = -\frac{\partial \log p_{\omega_{s,i}}(y \,|\, z = s, \widetilde{\mathbf{h}}_{s,i})}{\partial \widetilde{\mathbf{h}}_{s,i}} \cdot \nabla\widetilde{\mathbf{h}}_{s,i}$

% $\mathbf{d}_{\eta_{s,i}} = \sum_{k=1}^{S} \pi_{k,i} \frac{\partial \log\mathbb{P}_{\theta}(z=k|\cdot)}{\partial \widetilde{\mathbf{h}}_{s,i}} \cdot \nabla\widetilde{\mathbf{h}}_{s,i}$

% $\mathbf{g}_{\theta_{i}} = -\sum_{k=1}^{S} \pi_{k,i}  \frac{\partial \log\mathbb{P}(z=k|\cdot)}{\partial \theta_{i}}$

% % --
% original 

% $ \mathbf{g}_i = \begin{bmatrix} \pi_{s,i} \mathbf{g}_{\eta_{s,i}} + \mathbf{d}_{\eta_{s,i}} \\ \vdots \\ \pi_{s,i} \mathbf{g}_{\omega_{s,i}} \\ \vdots \\ \mathbf{g}_{\theta_{i}} \end{bmatrix} $

% $\nabla \mathcal{L}\left( \{\eta_{s,i}, \omega_{s, i}\}_{s=1}^S, \theta_i \right) = \mathbb{E}[\mathbf{g}_i]$

% % --
% lower bound 

% $\mathbf{\overline{g}}_i = \begin{bmatrix} \frac{1}{S}\mathbf{g}_{\eta_{s,i}} \\ \vdots \\ \frac{1}{S} \mathbf{g}_{\omega_{s,i}} \\ \vdots \\ \mathbf{0} \end{bmatrix}$

% $\nabla \overline{\mathcal{L}} \big( \{\eta_{s,i}, \omega_{s,i}\}_{s=1}^S \big) = \mathbb{E}[\mathbf{\overline{g}}_i]$

% $\mathring{\mathbf{g}}_i = \begin{bmatrix} \mathbf{g}_{\eta_{s,i}} \\ \vdots \\ \mathbf{g}_{\omega_{s,i}} \\ \vdots \\ \mathbf{0} \end{bmatrix}$

% % --
% \begin{align}
% & \mathbb{E}[\mathcal{L}\left( \{\eta_{s,i+1}, \omega_{s,i+1} \}_{s=1}^S, \theta_{i+1} \right)] - \mathbb{E}[\mathcal{L}\left( \{\eta_{s,i}, \omega_{s,i} \}_{s=1}^S, \theta_{i} \right)] \\
% \leq & 
% -\mu \langle \mathbb{E}[\mathbf{\overline{g}}_i], \mathbb{E}[\mathbf{g}_i] \rangle 
% +\frac{\mu^2 L}{2} \mathbb{E}[ \norm{\mathbf{\overline{g}}_i}^2 ] \\
% = & 
% -\frac{\mu}{S} \langle \mathbb{E}[\mathring{\mathbf{g}}_i], \mathbb{E}[\mathbf{g}_i] \rangle
% +\frac{\mu^2 L}{2S^2} \mathbb{E}[ \norm{\mathring{\mathbf{g}}_i}^2 ] \label{eq:theory_1}
% \end{align}

% where h·, ·i is the Euclidean inner product on tensor, dot product of two vectors 

% \begin{align}
% -\frac{\mu}{S} \langle \mathbb{E}[\mathbf{\mathring{g}}_i], \mathbb{E}[\mathbf{g}_i] \rangle = 
%  \frac{\mu}{2S} \big\lVert \mathbb{E}[\mathbf{\mathring{g}}_i] - \mathbb{E}[\mathbf{g}_i] \big\rVert^2
% -\frac{\mu}{2S} \big\lVert \mathbb{E}[\mathbf{\mathring{g}}_i] \big\rVert^2
% -\frac{\mu}{2S} \big\lVert \mathbb{E}[\mathbf{g}_i] \big\rVert^2
% \end{align}

% with $\norm{a+b}^2 \leq 2\norm{a}^2 + 2\norm{b}^2$

% \begin{align}
% \frac{\mu}{2S}\norm{\mathbb{E}[\mathbf{\mathring{g}}_i] - \mathbb{E}[\mathbf{g}_i]}^2 
% & = \frac{\mu}{2S} 
% \left\lVert 
% \mathbb{E}\begin{bmatrix} \mathbf{g}_{\eta_{s,i}} \\ \vdots \\ \mathbf{g}_{\omega_{s,i}} \\ \vdots \\ \mathbf{0} \end{bmatrix}
% - \mathbb{E}\begin{bmatrix} \pi_{s,i} \mathbf{g}_{\eta_{s,i}} + \delta_{\eta_{s,i}} \\ \vdots \\ \pi_{s,i} \mathbf{g}_{\omega_{s,i}} \\ \vdots \\ \mathbf{g}_{\theta_{i}} \end{bmatrix} \right\rVert^2 \\
% & = \frac{\mu}{2S} 
% \left\lVert 
% \mathbb{E}\begin{bmatrix} \mathbf{g}_{\eta_{s,i}} \\ \vdots \\ \mathbf{g}_{\omega_{s,i}} \\ \vdots \\ \mathbf{0} \end{bmatrix}
% - \mathbb{E} \begin{bmatrix} \pi_{s,i} \mathbf{g}_{\eta_{s,i}} \\ \vdots \\ \pi_{s,i} \mathbf{g}_{\omega_{s,i}} \\ \vdots \\ \mathbf{0} \end{bmatrix}  
% - \mathbb{E} \begin{bmatrix} \delta_{\eta_{s,i}} \\ \vdots \\ \mathbf{0} \\ \vdots \\ \mathbf{g}_{\theta_{i}} \end{bmatrix} 
% \right\rVert^2 \\
% & \leq \frac{\mu}{S} 
% \left\lVert 
% \mathbb{E}\begin{bmatrix} \mathbf{g}_{\eta_{s,i}} \\ \vdots \\ \mathbf{g}_{\omega_{s,i}} \\ \vdots \\ \mathbf{0} \end{bmatrix}
% - \mathbb{E} \begin{bmatrix} \pi_{s,i} \mathbf{g}_{\eta_{s,i}} \\ \vdots \\ \pi_{s,i} \mathbf{g}_{\omega_{s,i}} \\ \vdots \\ \mathbf{0} \end{bmatrix}
% \right\rVert^2
% + \frac{\mu}{S} 
% \left\lVert 
% \mathbb{E} \begin{bmatrix} \delta_{\eta_{s,i}} \\ \vdots \\ \mathbf{0} \\ \vdots \\ \mathbf{g}_{\theta_{i}} \end{bmatrix}
% \right\rVert^2
% \end{align}


% \begin{align}
% \frac{\mu}{S} 
% \left\lVert 
% \mathbb{E}\begin{bmatrix} \mathbf{g}_{\eta_{s,i}} \\ \vdots \\ \mathbf{g}_{\omega_{s,i}} \\ \vdots \\ \mathbf{0} \end{bmatrix}
% - \mathbb{E} \begin{bmatrix} \pi_{s,i} \mathbf{g}_{\eta_{s,i}} \\ \vdots \\ \pi_{s,i} \mathbf{g}_{\omega_{s,i}} \\ \vdots \\ \mathbf{0} \end{bmatrix}
% \right\rVert^2 
% \leq 
% \frac{\mu}{S} 
% \mathbb{E}[ \sum_{s=1}^S (\norm{\mathbf{g}_{\eta_{s,i}}}^2 + \norm{\mathbf{g}_{\omega_{s,i}}}^2) ] 
% = \frac{\mu}{S} \mathbb{E}\norm{\mathring{\mathbf{g}}_i}^2
% \end{align}

% assumption

% $\mathbb{E}[ \norm{\mathbf{g}_{\omega_{s,i}}}^2 ]$ $G^2$, $\zeta^2$

% $\mathbb{E}[ \norm{\mathbf{g}_{\eta_{s,i}}}^2 ]$

% $\mathbb{E}[ \norm{\mathbf{\delta}_{\eta_{i}}}^2 ]$

% $\mathbb{E}[ \norm{\mathbf{g}_{\theta_{i}}}^2 ]$

% \begin{align}
% (\ref{eq:theory_1}) 
% & \leq 
% \frac{\mu}{S}\mathbb{E}\norm{\mathring{\mathbf{g}}_i}^2 
% + \frac{\mu}{S} 
% \left\lVert 
% \mathbb{E} \begin{bmatrix} \mathbf{d}_{\eta_{s,i}} \\ \vdots \\ \mathbf{0} \\ \vdots \\ \mathbf{g}_{\theta_{i}} \end{bmatrix}
% \right\rVert^2
% -\frac{\mu}{2S}\norm{ \mathbb{E}[\mathbf{\mathring{g}}_i] }^2
% -\frac{\mu}{2S}\norm{ \mathbb{E}[\mathbf{g}_i] }^2 
% +\frac{\mu^2 L}{2S^2}\mathbb{E} \norm{\mathring{\mathbf{g}}_i}^2 \\
% & \leq
% \frac{\mu}{2S}\mathbb{E}\norm{\mathring{\mathbf{g}}_i}^2 
% + \frac{\mu}{2S}\mathbb{E}\norm{\mathring{\mathbf{g}}_i}^2
% -\frac{\mu}{2S}\norm{ \mathbb{E}[\mathbf{\mathring{g}}_i] }^2
% + \frac{\mu}{S} 
% \left\lVert 
% \mathbb{E} \begin{bmatrix} \mathbf{d}_{\eta_{s,i}} \\ \vdots \\ \mathbf{0} \\ \vdots \\ \mathbf{g}_{\theta_{i}} \end{bmatrix}
% \right\rVert^2
% -\frac{\mu}{2S}\norm{ \mathbb{E}[\mathbf{g}_i] }^2 
% +\frac{\mu^2 L}{2S^2}\mathbb{E} \norm{\mathring{\mathbf{g}}_i}^2 \\
% \end{align}

% \begin{align}
% & \mathbb{E}[\mathcal{L}\left( \{\eta_{s,i+1}, \omega_{s,i+1} \}_{s=1}^S, \theta_{i+1} \right)] - \mathbb{E}[\mathcal{L}\left( \{\eta_{s,i}, \omega_{s,i} \}_{s=1}^S, \theta_{i} \right)] \\
% \leq 
% & \mu\zeta^2 
% + \mu G^2
% -\frac{\mu}{2S}\norm{\mathbb{E}[\mathbf{g}_i]}^2 
% +\frac{\mu^2 L}{S}G^2 
% \end{align}

% \begin{align}
% \frac{1}{I+1} \sum_{i=0}^I \norm{\mathbb{E}[\mathbf{g}_i]}^2 
% \leq
% \frac{2S\mathbb{E}[\mathcal{L}\left( \Theta_{0} \right)] - \mathbb{E}[\mathcal{L}\left( \Theta_{I} \right)]}{\mu (I+1)} 
% + 2 (S \zeta^2 + S G^2 + \mu L G^2) 
% \end{align}

% $ 0 \leq \pi_{s,i} \leq 1$

% Summing these inequalities from t = 0 to t = T gives

% \end{proof}


% where $\Theta_i$ represents $[\{\eta_{s,i}, \omega_{s,i} \}_{s=1}^S, \theta_{i}]$
% of minimizing the loss function $\mathcal{L}\left( \{\eta_s, \omega_s\}_{s=1}^S, \theta \right)$ or $\mathcal{L}\left( \{\eta_s, \omega_s\}_{s=1}^S, \theta, \{\tau_s\}_{s=1}^S \right)$, 
% n and 
% $\forall \mathbf{g} \in \{ \mathbf{g}_{\omega_{s}}, \mathbf{g}_{\eta_{s}}, \mathbf{g}_{\theta_{i}} \}$  $\mathbb{E}[ \lVert \delta - \mathbb{E}[\delta] \rVert^2]$
% $\mathbb{E} \lVert \delta \rVert^2$
% A function f(x) : R is said to be Lipschitz-smooth with constant L if, f(x) has bounded gradients, 
% mean-squared error of our gradient samples from the
% true gradient is bounded
% Let the learning rate satisfies,
% it holds— in expectation over the stochasticity a
% partial update through the lower bound still make the full gradient of the original loss function converge to 
% Then, following the update of the component specific parameters $\overline{\mathcal{L}}\big( \{\eta_s, \omega_s\}_{s=1}^S \big)$


% The latent variable $z_t$ is a discrete random variable defined on the set of values $\{1, \cdots, S\}$, each of which represents the corresponding data source. The quantity $p_{\theta_s}(y_t | z_t = s, \mathbf{x}_{s, <t})$ models the predictive probabilistic density of the target based on the historical data $\mathbf{x}_{s, <t}$ from a certain source $s$. 
% The quantity\footnote{We indicate with $p_\theta$ probability densities and $\mathbb{P}_{\omega}$ probability mass functions.} $\mathbb{P}_{\omega}(z_t = s \, | \mathbf{x}_{1, <t}, \cdots, \mathbf{x}_{S, <t})$ characterizes a time-varying categorical distribution dependent on multi-source data.
% It adaptively adjusts the contribution of the data source specific density $p_{\theta_s}(y_t | z_t = s, \mathbf{x}_{s, <t})$ at each time step. Clearly, it holds
% $\sum_{s = 1}^{S}\mathbb{P}_{\omega}(z_t = s \, | \mathbf{x}_{1, <t}, \cdots, \mathbf{x}_{S, <t}) = 1$. 
% Finally, $\Theta \triangleq \{ \theta_1, \cdots, \theta_S, \omega \}$ represents the parameters in data source specific components and the latent variable's probability function, and it will be learned in the training phase discussed below. 

% The latent variable $z_t$ is a discrete random variable defined on the set of values $\{1, \cdots, S\}$, each of which represents the corresponding data source. The quantity $p_{\theta}(y_t | z_t = s, \mathbf{x}_{s, <t})$ models the predictive probabilistic density of the target based on the historical data $\mathbf{x}_{s, <t}$ from a certain source $s$. The quantity\footnote{We indicate with $p_\theta$ probability densities and $\mathbb{P}_{\omega}$ probability mass functions.} $\mathbb{P}_{\omega}(z_t = s \, | \mathbf{x}_{1, <t}, \cdots, \mathbf{x}_{S, <t})$ is time-varying dependent on multi-source data and  adaptively adjusts the contribution of the data source specific density $p_{\theta}(y_t | z_t = s, \mathbf{x}_{s, <t})$ at each time step. Clearly, it holds
% $\sum_{s = 1}^{S}\mathbb{P}_{\omega}(z_t = s \, | \mathbf{x}_{1, <t}, \cdots, \mathbf{x}_{S, <t}) = 1$. 
% Finally, $\theta$ and $\omega$ in Eq.~\ref{eq:joint} represent the parameters of the probabilistic functions, which are learned in the training phase discussed below. 



% We now specify in detail the mathematical formulation of each component in the temporal mixture model. The inference process we presented so far does not relies on any specific formulation of the model and thus it is flexible to different specifications. 
% Without loss of generality, we present the following model specification for cryptocurrency data of this paper's interest.

% To specify the model, we need to define the predictive density function of individual sources, i.e. $p_{\theta}(y_t | z_t = s, \mathbf{x}_{s, <t})$ and the probability function of latent variable, i.e. $\mathbb{P}_{\omega}(z_t = s \, | \mathbf{x}_{1, <t}, \cdots, \mathbf{x}_{S, <t})$.
% %In the following learning phase, training instances have to contain data of unified shape. 
% We make a general assumption for both these functions that data from different sources are taken within the same time window w.r.t. the target time step.
% We denote by $h$ the window length, i.e. the number of past time steps which enter in the conditional probabilities. 
% We assume that this value is the same for each source.
% Eq.~\ref{eq:joint} is thus simplified as:
% \begin{align}
% \begin{split}
% \prod_{t}^{}
% \sum_{z_t = 1}^{S}
% & p_{\theta}(y_t | z_t = s, \mathbf{x}_{s, (-h,t)}) \cdot \\
% & \mathbb{P}_{\omega}(z_t = s | \mathbf{x}_{1,  (-h,t)}, \cdots, \mathbf{x}_{S, (-h,t)}), 
% \end{split}
% \end{align}
% where $\mathbf{x}_{s, (-h,t)}$ represents the data from source $s$ within the time window from $t-h$ to $t-1$ and $\mathbf{x}_{s, (-h,t)} \in \mathbb{R}^{d_s \times h}$. 

% First, for $p_{\theta}(y_t | z_t = s, \mathbf{x}_{s, (-h,t)})$,
% we choose the Gaussian distribution.
% Since $\mathbf{x}_{s, (-h,t)} \in \mathbb{R}^{d_s \times h}$ is a matrix, we choose bi-linear regression to parameterize the mean and variance of the Gaussian distribution as follows: 
% \begin{gather}
% y_t | z_t = s, \mathbf{x}_{s,(-h, t)}, ~~~~~\theta \sim \mathcal{N}\big( \mu_s(\mathbf{x}_{s,(-h, t)} \big), \sigma_s^2(\mathbf{x}_{s,(-h, t)})) \\
% \mu_s(\mathbf{x}_{s,(-h, t)}) = L_{\mu, s}^{\top} \cdot \mathbf{x}_{s,(-h, t)} \cdot R_{\mu, s} + b_{\mu, s} \\
% \sigma_s^2(\mathbf{x}_{s,(-h, t)}) =  (L_{\sigma, s}^{\top} \cdot \mathbf{x}_{s,(-h, t)} \cdot R_{\sigma, s} + b_{\sigma, s} )^2,
% \end{gather}
% where $L_{\mu, s}$, $L_{\sigma, s} \in \mathbb{R}^{d_s}$ and $R_{\mu, s}$, $R_{\sigma, s} \in \mathbb{R}^{h}$. $b_{\mu,s}$, while $b_{\sigma,s} \in \mathbb{R}$ are bias terms. 
% %\textcolor{red}{Fabrizios comment from mail about Gaussian.}
% Note that the above parameters are data source specific and then the parameter set $\theta$ can be denoted by $\theta = \{ L_{\mu, s}, L_{\sigma, s}, R_{\mu, s}, R_{\sigma,s}, b_{\mu,s}, b_{\sigma,s} \}_{s=1}^S$.

% As a results, mean and variance on individual data source are defined as: $\mathbb{E}[{y}_{\tau} | \mathbf{x}_{s, <\tau}, \Theta_m] = \mu_s(\mathbf{x}_{s,(-h, t)})$ and
% $\text{Var}({y}_{\tau} | z_t = s, \mathbf{x}_{s, <\tau}, \Theta_m) = \sigma_s^2(\mathbf{x}_{s,(-h, t)})$. 
% Consequently, the mean and uncertainties in the inference phase can be explicitly calculated.

% Second, we choose for $\mathbb{P}_{\omega}(z_t = s | \mathbf{x}_{1,  (-h,t)})$ a multinomial logistic function:

% \begin{equation}\label{formula:softmax}
% \mathbb{P}_{\omega}(z_t = s | \mathbf{x}_{1,  (-h,t)}, \cdots, \mathbf{x}_{S, (-h,t)})=\frac{\exp(\, f(\mathbf{x}_{s, (-h, t)}) \, )}{ \exp( \, \sum_{k=1}^S f(\mathbf{x}_{k, (-h, t)}) \, )},
% \end{equation}

% \begin{equation}
% f(\mathbf{x}) =   L^{\top} \cdot \mathbf{x} \cdot R + b
% \end{equation}
% where $L,R\in {\mathbb R}^{d_s}$ and $b\in {\mathbb R}$ is a bias term 


% As for $p_{\theta_s}(y_t | z_t = s, \mathbf{x}_{s, (-h,t)})$, due to the non-negative nature of the volume in cryptocurrency exchange and its statistical properties~\cite{bauwens2008moments}, we choose the log-normal distribution to model $y_t$ as:

% \begin{align}
%     \ln y_t \, | z_t \text{=} s, \mathbf{x}_{s,(-h, t)} \, \sim \, \mathcal{N}\big( \mu_{t,s}, \sigma_{t,s}^2)
% \end{align}


% In the following, by deriving the conditional variance of the target in the Bayesian mixture manner, 
% we demonstrate that the total variance is decomposed into aleatoric and epistemic uncertainties, which reflect different aspects of the variance of the target ${y}_{\tau}$.


% where $\omega_m$ is from sample $\Theta_m$.
% Eq.~\ref{eq:var} bridges the aleatoric and epistemic uncertainty by the derivation of total variance of ${y}_{\tau}$ in the Bayesian mixture setting.
% The decomposition in Eq.~\ref{eq:var} also
% theoretically demonstrates the relation between total variance and the aleatoric and epistemic uncertainty in Bayesian modeling, namely the total variance is composed of inherent noise and model uncertainty on the target.

% The aleatoric part in Eq.~\ref{eq:var} stems from variance induced from multi-source data. 
% It captures the noise inherent to the target which could depend on $\mathbf{x}_{s, < \tau}$.
% As a comparison, a classical aleatoric uncertainty (or volatility) estimation model, the GARCH, is typically used to estimate the volatility solely with the target time series.
% It has no mechanism to capture the evolving relevance of multi-source data to the aleatoric uncertainty of the target.  

% The epistemic uncertainty on mean in Eq.~\ref{eq:var} accounts for uncertainty in the model parameters i.e. uncertainty which captures our ignorance about which model generated our collected data.
% This uncertainty can be reduced when enough data are available, and is often referred to as model uncertainty.

% Then, in the experiment section, we will quantitatively examine the relation between the uncertainty score and prediction errors, and suggest the potential of the uncertainty score as an indicator of the prediction error levels during inference.

% commonly used aleatoric uncertainty
% Predictive uncertainty reflects the confidence of the model over the prediction. 

% It is valuable extra information for model interpretability and reliability.

% they provide information about their own accuracy and reliability.

% fall short in giving useful estimates of their predictive uncertainty. 

% Quantifying uncertainty is especially critical in real-world settings, which often involve input distributions that are shifted from the training distribution due to a variety of factors including sample bias and non-stationarity

% The uncertainty score in Eq.~\ref{eq:var} takes into account both the magnitude and level of the fluctuation in the target predictions. 




% . Having only a single tuneable parameter, temperature scaling cannot learn to act  on different class
% Temperature scaling is commonly used in settings such as knowledge distillation (Hinton et al., 2015) and statistical mechanics (Jaynes, 1957). 
% To the best of our knowledge, we are not aware of any prior use in the context of calibrating probabilistic models.
% The model is equivalent to maximizing the entropy of the output probability distribution subject to certain constraints on the logits



% prediction interval
% \begin{align}
% q(\alpha) = P^{-1}\left(\, y_t \,\Big|\, \{\mathbf{x}_{s,<t}\}_{s=1}^{S} \right)
% % = \sum_{s = 1}^{S} \mathbb{P}(z_t = s \,|\, \cdot ) \, P(y_t \, | \, z_t = s, \mathbf{h}_s)
% \end{align}
% where $\alpha \in (0, 1)$ and $P\left(\, y_t \,\Big|\, \{\mathbf{x}_{s,<t}\}_{s=1}^{S} \right) = \sum_{s = 1}^{S} \mathbb{P}(z_t = s \,|\, \cdot ) \, P(y_t \,|\, z_t = s, \mathbf{\widetilde{h}}_s)$



-------------------



\newpage
\section{Problem and Proposed Models}\label{sec:model}

\subsection{Problem Statement}

Let $y_t$ be the value from the target time series at time $t$.
Given $S$ number of different data sources, denote by $s \in \{1, \cdots, S\}$ the data source index. 
Then, the multi-source data used to predict $y_t$ are represented by $\{\mathbf{x}_{s,<t}\}_{s=1}^{S}$, where $\mathbf{x}_{s,<t}$ is the multi-dimensional time series data from a limited window of historical data of source $s$ prior to time $t$.
We assume $\{\mathbf{x}_{s,<t}\}_{s=1}^{S}$ could have different dimensions of variables/features and window lengths across sources and for simplicity, we skip the notations for time series window length and feature dimensions.
% $p(\, y_t \,|\, \{\mathbf{x}_{s,<t}\}_{s=1}^{S})$.

Also note that in this paper, for simple presentation, we assume that $\{\mathbf{x}_{s,<t}\}_{s=1}^{S}$ implicitly contains the historical data of the target variable $y_{<t}$ if available, either as an additional source or being included into a data source.


% We assume that there is access to a historical dataset
% However, we argue that learning from a single time series while useful in cases where indeed only one time-series is available 
% may not be optimal in settings where datasets contain multiple time-series, the shared patterns of which could potentially be exploited (Figure 1, right)
% A forecasting model capable of capturing the time-varying relevance of the multi-source data to the target variable
% We address the task of discrete-time multivariate time-series prediction, with the goal of forecasting multiple time-steps ahead. 
% The model developed below is flexible to consume multi-source data of arbitrary number of sources and dimensionalities of individual source data.
% We assume that there is access to a historical dataset for training, but after training the model must perform prediction based on a limited window of historical data.
% For simplicity, we will use one data sample of the target $y_t$ to present the proposed model.
% In reality, the training, validation, and testing data contain the samples collected in a time period.
% More quantitatively, the generative process of the target variable $y_t$ conditional on multi-source data $\{\mathbf{x}_{1,t}, \cdots, \mathbf{x}_{S,t}\}$ is formulated as the following probabilistic mixture process:
% \begin{align}
% \label{eq:joint}
% p(\, y_t \,|\, \{\mathbf{x}_{s,<t}\}_{s=1}^{S} )
% \end{align}
% is a probability distribution parameterized by. 
% In our experiments, G is a normal distribution with mean and constant diagonal varian (Stochastic Latent Residual Video Prediction)
% As d is fixed, we will abbreviate dk=1 x k by k x k throughout.
% Formally, given a source sentence x and reference translation y, a mixture model introduces a multinomial latent variable % z ∈ {1, · · · , K}, 
% and decomposes the marginal likelihood as:



\subsection{Model Structures}
% \textbf{[key elements]: disentangled representations, temperature scaling in the gate function, }

Specifically, define a discrete random variable $z_t$ on the data source index set i.e. $z_t \in \{1, \cdots, S\}$, which will be used to decompose the dependence on multi-source data.
In the context of deep learning based forecasting, a continuous hidden representation is normally learned from the input data and then used as the predictive feature to subsequent models.
In our case, denote by $\mathbf{h}_{s,t}$ the predictive hidden representation learned from data source $\mathbf{x}_{s,<t}$.

Next, by introducing the discrete random variable $z_t$ and the predictive hidden representations $\{\mathbf{h}_s\}_{s=1}^S$ as latent variables into the probability model of $y_t$, the factorization of the joint distribution is formulated as follows:
\begin{align}\label{eq:overall_model}
% & p(\, y_t \,|\, \{\mathbf{x}_{s,<t}\}_{s=1}^{S} ) = 
\int \sum_{s=1}^S 
\underbrace{\mathbb{P} \Big(z_t=s \,\Big|\, \cdot \Big)}_{\text{weight module}} 
\underbrace{p \Big( y_t \,\Big|\, z_t=s, \mathbf{h}_{s,t} \Big)}_{\text{prediction module}} 
\underbrace{p \Big(\mathbf{h}_{s,t} \,\Big|\, \mathbf{x}_{s,<t} \Big)}_{\text{representation module}}
\text{d}\mathbf{h}_{1:S,t}
\end{align}
In Eq.~(\ref{eq:overall_model}), we have one degree of freedom on the weight module and will present two specific designs in the following.
$z_t$ is a multinomial random variable satisfying $\sum_{s=1}^S \mathbb{P}(z_t=s|\cdot) = 1$, and its probability function $\mathbb{P}(z_t=s|\cdot)$ serves as the time-varying weight of each data source's contribution to the overall density function.
Each data source has the corresponding prediction model using the representation learned from time series data.

As for the degree of freedom on $\mathbb{P}(z_t=s \,|\, \cdot )$, we will present the proposed \textit{Sharing} and \textit{Residual} realizations.
There are potentially others ways of specifying the weight module, but in this work we focus on investigating these two fundamental ones which could inspire the future work.

The \textit{Sharing} realization is based on the idea of using the predictive representations $\{\mathbf{h}_i\}_{i=1}^S$ as the input features into the weight module. 
To this end, after pooling the predictive representations of data sources and re-arranging the terms in Eq.~(\ref{eq:overall_model}), the join distribution is expressed as: 
\begin{align}\label{eq:share}
\int p\Big( \{\mathbf{h}_{s,t}\}_{s=1}^S \,\Big|\, \{ \mathbf{x}_{s,<t} \}_{s=1}^{S} \Big)
\sum_{s = 1}^{S} 
\mathbb{P}(z_t = s \,|\, \{\mathbf{h}_{i,t}\}_{i=1}^S )\, p(y_t \,|\, z_t = s, \mathbf{h}_{s,t}) \text{d}\mathbf{h}_{1:S,t}
\end{align}

The \textit{Residual} realization is intended for providing supplementary representations for the weigh module, given that besides the predictive representation, there could be residual information left in data sources and useful for the weigh module~\cite{?}.
Meanwhile, in the following, we will show this residual weight module implicitly amounts to being equipped with a learnable temperature scaling mechanism.

Concretely, by introducing another set of data source specific residual representations denoted by $\{\mathbf{r}_{s,t}\}_{s=1}^S$, the weight module now makes use of two complementary sets of representations, thereby leading to the factorization as follows:
\begin{align}\label{eq:resi}
\begin{split}
& \int\int p\Big( \{\mathbf{h}_{s,t}\}_{s=1}^S, \{\mathbf{r}_{s,t}\}_{s=1}^S \,\Big|\, \{ \mathbf{x}_{s,<t} \}_{s=1}^{S} \Big) \cdot 
\\
& \sum_{s = 1}^{S} 
\mathbb{P}(z_t = s \,|\, \{\mathbf{h}_{i,t}\}_{i=1}^S, \{\mathbf{r}_{i,t}\}_{i=1}^S )\, p(y_t \,|\, z_t = s, \mathbf{h}_{s,t})  \text{d}\mathbf{h}_{1:S,t} \text{d}\mathbf{r}_{1:S,t}
\end{split}
\end{align}


In the next, we will elaborate on each module's specification. 

\textbf{Weight Module.}
In the \textit{Sharing} version, the weight module is defined by the softmax function as follows:
\begin{align}\label{eq:softmax_s}
\mathbb{P}_{\theta}(z_t = s \,|\, \{\mathbf{h}_i\}_{i=1}^S ) & \triangleq \frac{\exp(\, f_{\theta_s}(\mathbf{h}_s) \, )}{ \sum_{i=1}^S\exp(\,  f_{\theta_i}(\mathbf{h}_i) \,)}
\end{align}
where $\theta_{s}$ denote the parameters of the logit function for data source $s$, i.e. $f_{\theta_s}( \cdot ): \mathbb{R}^{d_s} \rightarrow \mathbb{R}$, where $d_s$ is the dimensionality of input vectors. 
$f_{\theta_s}( \cdot )$ can be any flexible function such as neural networks.
Denote by $\theta = \{\theta_{s}\}_{s=1}^{S}$ the set of trainable parameters in the weight module, since it will be jointly learned. 

In the \textit{Residual} version, the residual representations $\{\mathbf{r}_s\}_{s=1}^S$ are integrated as follows:
\begin{align}
\mathbb{P}_{\theta}(z_t = s \,|\, \{\mathbf{h}_s\}_{i=1}^S, \{\mathbf{r}_s\}_{i=1}^S ) 
& \triangleq \frac{\exp(\, f_{\theta_s}(\mathbf{h}_s) +f_{\theta_s}(\mathbf{r}_s) \,)}{\sum_{i=1}^S\exp(\, f_{\theta_i}(\mathbf{h}_i)+f_{\theta_i}(\mathbf{r}_i) \,)} 
 = \frac{\exp(\, f_{\theta_s}(\mathbf{h}_s) \,)/T_s }{\sum_{i=1}^S\exp(\,  f_{\theta_i}(\mathbf{h}_i) \,)/T_i} \label{eq:temp_scale}
\end{align}
, where $T_s \triangleq \exp(-f_{\theta_s}(\mathbf{r}_s))$.

In the context of the phased learning presented in the next section, compared to Eq.~(\ref{eq:softmax_s}), Eq.~(\ref{eq:temp_scale}) can be considered as a kind of temperature scaling~\cite{?}.
This is because the residual representations are learned in the latter phase than the predictive representations, and thus they serve to incrementally adjust the softmax components derived from predictive representations, i.e. $\exp(\, f_{\theta_i}(\mathbf{h}_i) \,)$, through $T_i$.



\textbf{Prediction Module.} Given the predictive representations $\{\mathbf{h}_{s,t}\}_{s=1}^S$, this module generates the data source-wise predictive density function of $y_t$.
In this paper, we focus on two types of distributions depending on the domain of $y_t$, namely, normal distribution for $y_t \in \mathbb{R}$, and log-normal distribution for $y_t \in \mathbb{R}^{+}$, while the forecasting mixture allows for flexible specifications of the target distribution. 

In particular, the density function $p(y_t \, | \, z_t = s, \mathbf{h}_s)$ is formulated as:
\begin{align}
\text{Normal: } y_t | \mathbf{h}_{s,t} \sim \mathcal{N}(\mu_{t,s}, \sigma_{t,s}^2) 
\,\text{ or }\,  \\
\text{Log-normal: } \log y_t \, | \mathbf{h}_{s,t} \sim \mathcal{N}(\mu_{t,s}, \sigma_{t,s}^2)
\end{align}
, where $\mu_{t,s}, \sigma_{t,s}^2 = g_{\omega_s}(\mathbf{h}_{s,t})$, and $g_{w_s}(\mathbf{h}_{s,t})$ can be any flexible function such as multi-layer dense networks parameterized by $\omega_s$.
Overall, we have the set of learnable parameters $\{\omega_s\}_{s=1}^S$ in the prediction module.

\textbf{Representation Module.}
There are a variety of probabilistic representation learning methods for time series data, e.g. neural networks based state-space models, variational and stochastic recurrent neural networks, etc~\cite{?}. 
Since advancing the representation learning is not the focus of this paper, we choose a simple way to formulate the representation module, i.e. placing a Dirac delta distribution centered at the output of a temporal data encoder \cite{fraccaro2016sequential,karl2016deep}, as follows: 
\begin{align}
p\Big( \{\mathbf{h}_s\}_{s=1}^S \, \Big| \, \{ \mathbf{x}_{s,<t} \}_{s=1}^{S} \Big) = \prod_{s=1}^S \delta(\mathbf{h}_s - \widetilde{\mathbf{h}}_s) \\
\text{  }\text{  }  \text{ s.t. } 
\widetilde{\mathbf{h}}_s = \text{NN}_{\eta_s}(\mathbf{x}_{s, <t}), \forall s = 1, \cdots, S
\end{align}
, where $\text{NN}_{\eta_s}(\mathbf{x}_{s, <t})$ is the encoder to model the temporal dynamics of data source $s$ and $\eta_s$ denotes the trainable parameters in it.
In this paper, we employ the LSTM architecture to encode each source's time series data.

If it is hypothesized to there exist a global latent factor governing the dynamics across data sources, above formulation is extensible by learning a global representation from all data sources and sharing it across individual predictive representations~\cite{?}.
This would lead to a formulation expressed as: 
$ p( \{\mathbf{h}_s\}_{s=1}^S, \mathbf{h}_0 \,|\, \{ \mathbf{x}_{s,<t} \}_{s=1}^{S} ) = \prod_{s=1}^S p( \mathbf{h}_s \,|\, \mathbf{h}_0, \mathbf{x}_{s,<t} ) \cdot p( \mathbf{h}_0 \,|\, \{\mathbf{x}_{s,<t}\}_{s=1}^S ) $, where $\mathbf{h}_0$ denotes the global representation.
The further exploration and evaluation of this idea would be the future work.

Likewise, in the \textit{Residual} mixture, the representation module is expressed as:
\begin{align}
& p\Big(\{\mathbf{h}_s\}_{s=1}^S, \{\mathbf{r}_s\}_{s=1}^S \, \Big| \, \{ \mathbf{x}_{s,<t} \}_{s=1}^{S} \Big) = \prod_{s=1}^S \delta(\mathbf{h}_s - \widetilde{\mathbf{h}}_s) \cdot \delta(\mathbf{r}_s - \widetilde{\mathbf{r}}_s) \\
& \text{  }\text{  }  \text{ s.t. }
\widetilde{\mathbf{h}}_s = \text{NN}_{\eta_s}(\mathbf{x}_{s, <t}), \text{  }\text{  } 
\widetilde{\mathbf{r}}_s = \text{NN}_{\tau_s}(\mathbf{x}_{s, <t}), \text{  } 
\forall s = 1, \cdots, S
\end{align}
% , given the covariates of the next time point ct, via the updated hidden state ht1:
% (Autoregressive Denoising Diffusion Models for Multivariate Probabilistic Time Series Forecasting)
% \underline{Future work}, common factors
% discuss: common factors, either added into individual representation, or another new component model

Overall, the trainable parameter set is $\{\eta_s \}_{s=1}^S$ for the \textit{Sharing} mixture, and $\left(\{\eta_s \}_{s=1}^S, \{\tau_s\}_{s=1}^S \right)$ for the \textit{Residual} one.



\section{Inference and Learning}
% In this section, we first present some favorable properties of the inference, and then the learning process.

\subsection{Inference}
% \textbf{[key elements]: adaptive point and quantile prediction, uncertainty quantification, }
Given the learned parameters, a variety of predictive quantities can be derived from the resulting multi-modal distribution of the target variable as in Eq.~\ref{eq:overall_model}.
In the following, we will mainly present the point prediction and associated uncertainty score. 
In the experiment section, we will additionally evaluate the likelihood and quantile prediction related performance.

For simplicity, we will express the weight module as $\mathbb{P}_{\theta}(z_{t} = s \,|\, \cdot )$, when differentiating the \textit{Sharing} and \textit{Residual} formations makes no difference for the presentation.

\textbf{Point Predictions.}
It is denoted by $\hat{y}_t$ and defined by the predictive mean of the mixture.
Based on the data dependent weights capturing the varying contribution of each data source, it is expressed as:
\begin{align}\label{eq:mean}
\hat{y}_t \triangleq \mathbb{E}[y_t \,|\, \{\mathbf{x}_{s, <t}\}_{s=1}^S] = \sum_{s=1}^S & \mathbb{P}_{\theta}(z_{t} = s \,|\, \cdot ) \cdot \mathbb{E}[{y}_{t} \,|\, z_t=s, \widetilde{\mathbf{h}}_s]
\end{align}
, where $\mathbb{E}[{y}_{t} \,|\, z_t=s, \widetilde{\mathbf{h}}_s ]$ denotes the predictive mean by individual sources. 
As is defined in the prediction module, it is $\mu_{t,s}$ for normal distribution and $\exp(\mu_{t,s} + \frac{1}{2}\sigma_{t,s}^2)$ for the log-normal distribution~\cite{?}. 


\textbf{Uncertainty.}
In a forecasting task, the predictive variance is commonly used as an uncertainty measure to reflect the reliability of the prediction \cite{}.
In our case, the uncertainty $u_t$ is defined as:
\begin{align}\label{eq:var}
\begin{split}
& u_t \triangleq \text{Var}(\, {y}_{t} \,|\, \{\mathbf{x}_{s, <t}\}_{s=1}^S ) = \underbrace{ \sum_{s = 1}^S \mathbb{P}_{\theta}(z_t = s \,|\, \cdot) \text{Var}(y_t \,| z_t = s, \widetilde{\mathbf{h}}_s) }_{\text{Aleatoric Uncertainty}} + \\
& \underbrace{ \sum_{s = 1}^S \mathbb{P}_{\theta}(z_t = s \,|\, \cdot) \mathbb{E}^2[y_t \,|\, z_t=s, \widetilde{\mathbf{h}}_s ] - \mathbb{E}^{2}[y_t \,|\, \{\mathbf{x}_{s, <t}\}_{s=1}^S ]}_{\text{Mixture Uncertainty}}
\end{split}
\end{align}
, where $\text{Var}(y_t \,| z_t = s, \widetilde{\mathbf{h}}_s)$ is aforementioned $\sigma_{t,s}^2$ for normal distribution and $\exp(\sigma_{t,s}^2 -1) \cdot \exp(2 \mu_{t,s} + \sigma_{t,s}^2)$ for log-normal distribution~\cite{?}.

Noticeably, the uncertainty score in Eq.~\ref{eq:var} is uniquely derived from two components both relying on the weights.
The aleatoric uncertainty quantifies the predictive noise inherent in the target, which could be captured through multi-source data.
The mixture uncertainty reflects the variation among each data source's predictions.

As a comparison, the uncertainty quantification methods in existing works (e.g. Bayesian and stochastic neural networks, ensemble methods, etc.) mostly utilize equal-weighted samples of model parameters or latent states~\cite{?}.
Meanwhile, it is feasible to incorporate the model uncertainty by sampling from the (approximate) posterior distribution of model parameters or deep ensembles and this would be in the future work.  

In the following, we first give a qualitative example of interpreting the uncertainty score. 
Then, in the experiment section, we will quantitatively examine the relation between the uncertainty score and prediction errors, and suggest the potential of the uncertainty score as an indicator of the prediction error levels during inference.

For instance, in the middle panel of Fig.~\ref{fig:example}(b), the example period \circled{1} has high aleatoric uncertainty, and accordingly in the top panel, the prediction values fluctuate in the corresponding time period of \circled{1}.
Because these noisy values are mostly located on the relatively low level of the target value range, and all data sources are able to provide the predictions covering that level, the mixture uncertainty is relatively low in \circled{1}.

On the contrary, as for the example period \circled{2}, the prediction has small aleatoric uncertainty, thereby fluctuating with small magnitudes, as is shown in the top panel. 
However, the prediction values mainly distribute on the high level of the target domain, and it is likely that only few data sources are able to provide predictions on that level, and therefore the mixture uncertainty is high.
Meanwhile, the resulting high overall uncertainty score raises the awareness of potentially increasing prediction errors on that level.




% commonly used aleatoric uncertainty
% Predictive uncertainty reflects the confidence of the model over the prediction. 
% It is valuable extra information for model interpretability and reliability.
% they provide information about their own accuracy and reliability.
% fall short in giving useful estimates of their predictive uncertainty. 
% Quantifying uncertainty is especially critical in real-world settings, which often involve input distributions that are shifted from the training distribution due to a variety of factors including sample bias and non-stationarity
% The uncertainty score in Eq.~\ref{eq:var} takes into account both the magnitude and level of the fluctuation in the target predictions. 


\subsection{Issues with the straightforward training}

yet still incompletely understood,

Training forecasting models is often formulated into the Empirical Risk Minimization (ERM) framework.
$\mathcal{D} = \big\{ y_t, \{\mathbf{x}_{s,<t}\}_{s=1}^{S} \big\}_{t \in \mathcal{T}}$, where $\mathcal{T}$ represents the set of timestamps at which the data instances are collected.

We consider the training of a non-convex loss function f : Rd → R. 

\textbf{Loss functions}
Thus, the integral over the hidden states is replaced by a single point; we make the dependency of ht on both 
% z1:t and x1:t explicit

\begin{align}
& \mathcal{L}\left(\{\eta_s, \omega_s \}_{s=1}^S, \theta \,; \mathcal{D} \right) 
= \frac{1}{|\mathcal{T}|} \sum_{t \in \mathcal{T}} 
\left[-\log \sum_{s = 1}^{S} \mathbb{P}_{\theta}(z_t = s \,|\, \{\widetilde{\mathbf{h}}_{i,t}\}_{i=1}^S) \, p_{{\omega}_{s}}(y_t \,|\, z_t = s, \widetilde{\mathbf{h}}_{s,t}) \right] 
\end{align}
where $\widetilde{\mathbf{h}}_{s,t} = \text{NN}_{\eta_s}(\mathbf{x}_{s, <t}) $


\begin{equation}
\mathcal{L}\left(\{\eta_s, \omega_s\}_{s=1}^S, \theta, \{\tau_s\}_{s=1}^S \,; \mathcal{D} \right) 
= \frac{1}{|\mathcal{T}|} \sum_{t \in \mathcal{T}} 
\left[-\log \sum_{s = 1}^{S} \mathbb{P}_{\theta}(z_t = s \,|\, \{ \mathbf{\widetilde{h}}_{i,t} \}_{i=1}^S, \{\mathbf{\widetilde{r}}_{i,t}\}_{i=1}^S ) \, p_{{\omega}_{s}}(y_t \,|\, z_t = s, \widetilde{\mathbf{h}}_{s,t}) \right]
\end{equation}
where $\widetilde{\mathbf{h}}_{s,t} = \text{NN}_{\eta_s}(\mathbf{x}_{s, <t}) $ and $\widetilde{\mathbf{r}}_{s,t} = \text{NN}_{\tau_s}(\mathbf{x}_{s, <t}) $

For most training of deep neural networks, SGD or its
variants are used to optimize such loss functions. At
every step t of training, a mini-batch of training examples
% {(xi, yi), 1 ≤ i ≤ n} 
is sampled, where n is the mini-batch
size, n N. Then the parameters are adjusted according to
the descent direction of the expected loss on the mini-batch.
Let’s consider vanilla SGD:

A stochastic gradient optimizer refers to an iterative algorithm that repeatedly updates model parameters with a uniformly sampled minibatch of training examples. 
Concretely, this stochastic gradient with mini-batch size M is computed as follows:


For any iterative stochastic gradient optimizer 

We assume for a weight vector  to have access to a stochastic gradient 
% g(w) ∈ Rd such that E[g(w)] = ∇f(w). 

This corresponds to the standard machine learning setting with g(w) representing a (mini-batch) gradient
of one (or several) components of the loss function. Stochastic Gradient Descent (SGD) computes a
sequence of iterates by the update rule

$\nabla \mathcal{L} \big( \{\eta_{s}, \omega_{s}\}_{s=1}^S, \theta \,;\, \mathcal{D} \big) = \mathbb{E}_t[\mathbf{g} ]$

$t$ represent the sample instance. 

$\mathbf{g} = \nabla \mathcal{L} \big( \{\eta_{s,i}, \omega_{s,i}\}_{s=1}^S, \theta_i \,;\, y_t, \{\mathbf{x}_{s,<t}\}_{s=1}^{S} \big)$

Without the loss of generality, in the proof we treat the mini-batch
M = 1.

the mini-batches. At each iteration, we assume access to an unbiased stochastic gradient 
% E[g(x)] = ∇f(x, ξ) 
corresponding to the paramet

The loss function that corresponds to the i-th
data sample is denoted by 
% `i
% : R
% d → R for i = 1, . . . , n

\textbf{[key elements]: imbalance and unstable issue in straightforward training, phased learning, }

intertwined effect

poor convergence, fail to, incompletely make fully use of individual source predictive power, overall performance on different metrics

we develop some intuition for this phenomenon.

misleadingly weight 


\begin{figure*}[!htbp]
\centering
\includegraphics[width=0.99\textwidth]{figures/tr_behavior.pdf}
\caption{ (a) Direct (b) ELBO (c) phased training, \tian{(c)} error bar by 5 runs, zoom in}
\label{fig:overeiw}
\end{figure*}



\tian{even if some data sources are redundant}



\textbf{Direct}

gradient EM

\begin{align}
\begin{split}
- \sum_{s = 1}^{S} \pi_{s, t} \nabla \log\big[ p_{{\omega}_{s}}(y_t \,|\, z_t = s, \widetilde{\mathbf{h}}_{s,t}) \, \mathbb{P}_{\theta}(z_t = s \,|\, \cdot) \big]
\end{split}
\end{align}

\begin{equation}\label{eq:weight}
\pi_{s, t} 
= p(z_t = s \,|\, y_t, \{\mathbf{x}_{s,<t}\}_{s=1}^{S}) 
= \frac{p_{{\omega}_{s}}(y_t \,|\, z_t = s, \widetilde{\mathbf{h}}_{s,t}) \, \mathbb{P}_{\theta}(z_t = s \,|\, \cdot)}{\sum_{k = 1}^{S} p_{{\omega}_{k}}(y_t \,|\, z_t = k, \widetilde{\mathbf{h}}_{k,t}) \, \mathbb{P}_{\theta}(z_t = k \,|\, \cdot)}
\end{equation}

assume the prior are roughly equal, the weights guide the learning of individual source's models

premature weighting

hardly reflect the predictive power of each data source 

$\pi_{s, t}$ is the posterior weight. 

$\mathcal{L}\left(\{\eta_s, \omega_s\}_{s=1}^S, \theta \right)$

$\mathcal{L}\left(\{\eta_s, \omega_s\}_{s=1}^S, \theta, \{\tau_s\}_{s=1}^S \right)$


\textbf{ELBO training}

strict lower bound

\begin{equation}
- \sum_{s = 1}^{S} \nabla \left[ \mathbb{P}_{\theta}(z_t = s \,|\, \cdot) \, \log p_{{\omega}_{s}}(y_t \,|\, z_t = s, \widetilde{\mathbf{h}}_{s,t}) \right]
\end{equation}

correct the prior 

\subsection{Phased learning}

In the following, We first present the observation which motivates the proposal of the phased learning method. 

\begin{lemma}\label{theo:bound_loss}
In either sharing or residual mode of the mixture model, let $\Theta$ represent the entire set of model parameters, 
i.e. $\Theta = \left\{ \{\eta_s, \omega_s\}_{s=1}^S, \theta \right\}$ or $\Theta = \left\{ \{\eta_s, \omega_s\}_{s=1}^S, \theta, \{\tau_s\}_{s=1}^S \right\}$.
At any point of $\Theta$, there exists the following upper bound of the corresponding loss function: 
\begin{equation}
\mathcal{L}\left( \Theta \right) \leq 
\overline{\mathcal{L}} \big( \{\eta_s, \omega_s\}_{s=1}^S \big)
\triangleq -\sum_{s = 1}^{S} \frac{1}{S} \log p_{\omega_s}(y_t \,|\, z_t = s, \widetilde{\mathbf{h}}_{s,t})
\end{equation}
where
% $\overline{\mathcal{L}}\big( \{\eta_s, \omega_s\}_{s=1}^S \big) = - \sum_{s = 1}^{S} \frac{1}{S} \log  p_{\omega_s}(y_t \,|\, z_t = s, \widetilde{\mathbf{h}}_{s,t} ), \text{  }$
$\widetilde{\mathbf{h}}_{s,t} = \text{NN}_{\eta_s}(x_{s, <t})$
\end{lemma}


The right hand side of Eq.~\ref{eq:bound} depends on the component specific parameter.



If we minimize the upper bound of the loss function, the parameter set $\{\eta_s, \omega_s\}_{s=1}^S$ will be updated through the gradient of the first term on the right hand side. 
Then, the bound constantly holds, regardless of updating the rest of parameters of the original loss function. 

This ensures that all parameters are optimised individually to their best possible extent instead
of down-weighting less informative so



requiring artificial subsampling of the observations to ensure that
the individual modalities are learnt faithfull

\tian{Neutral phase, impartial phase, collective}

Component phase: $ \overline{\mathcal{L}}\big( \{\eta_s, \omega_s\}_{s=1}^S \big) $, the component specific parameters

Global phase: $ \mathcal{L}\left( \Theta \right) $, the component specific parameters, Then, when the learning switch to the global phase,  all parameters are jointly updated to minimize the overall loss function








In stochastic gradient decent style training, given a random training sample, the vectorized derivative of the component model w.r.t. the prediction and representation parameters are defined as:
\begin{equation}
\mathbf{g}_{\omega_{s}} \triangleq -\frac{\partial \log p_{\mathbf{\omega}_{s}}(y_t \,|\, z_t = s, \widetilde{\mathbf{h}}_{s,t})}{\partial \omega_{s}}
\end{equation}
\begin{equation}
\mathbf{g}_{\eta_{s}} \triangleq -\frac{\partial \log p_{\omega_{s}}(y_t \,|\, z_t = s, \widetilde{\mathbf{h}}_{s,t})}{\partial \widetilde{\mathbf{h}}_{s,t}} \cdot \nabla\widetilde{\mathbf{h}}_{s,t}
\end{equation}


jacobia matrix to explain gradient update


\begin{lemma}\label{lemma:bound}
% Let $ \mathbf{d}_{\eta_{s}} \triangleq \sum_{k=1}^{S} \pi_{k,t} \frac{\partial \log\mathbb{P}_{\theta}(z_{t} = k | \cdot)}{\partial \widetilde{\mathbf{h}}_{s,t}} \cdot \nabla\widetilde{\mathbf{h}}_{s,t} $
In the component and global phase, the stochastic gradient used to update the individual data source's forecasting and representation parameters are respectively formulated as:
\begin{minipage}{0.47\textwidth}
\begin{align*}
\text{Component phase: } \frac{1}{S}\mathbf{g}_{\omega_{s}}, and \text{ } \frac{1}{S}\mathbf{g}_{\eta_{s}}  
\end{align*}
% \equationset{Component phase}\label{eqset:1}
\end{minipage}
%\hfill\vline
\hfill
\begin{minipage}{0.5\textwidth}
\begin{align*}
\text{Global phase: } \pi_{s,t}\mathbf{g}_{\omega_{s}}, and \text{ } \pi_{s,t} \mathbf{g}_{\eta_{s}} + \mathbf{d}_{\eta_{s}}
\end{align*}
% \equationset{Global phase}\label{eqset:2}
\end{minipage}
where $\pi_{s,t}$ is defined as in Eq.~\ref{eq:weight} and $\mathbf{d}_{\eta_{s}} \triangleq \sum_{k=1}^{S} \pi_{k,t} \frac{\partial \log\mathbb{P}_{\theta}(z_{t} = k | \cdot)}{\partial \widetilde{\mathbf{h}}_{s,t}} \cdot \nabla\widetilde{\mathbf{h}}_{s,t}$

\end{lemma}


% \begin{equation}
% \frac{1}{S} \mathbf{g}_{\omega_{s}} \text{ and } \pi_{s,t}\mathbf{g}_{\omega_{s}} 
% \end{equation}

% \begin{equation}
% \text{Component phase: } \frac{1}{S} \mathbf{g}_{\omega_{s}}, \frac{1}{S} \mathbf{g}_{\eta_{s}} \text{  } 
% \text{Global phase: } \pi_{s,t}\mathbf{g}_{\omega_{s}} , \pi_{s,t} \mathbf{g}_{\eta_{s}} + \mathbf{d}_{\eta_{s}}  
% \end{equation}

% \begin{minipage}{0.47\textwidth}
% \begin{align}
% \text{Component phase } \frac{1}{S} \mathbf{g}_{\omega_{s}},    \pi_{s,t}\mathbf{g}_{\omega_{s}}
% \end{align}
% % \equationset{Component phase}\label{eqset:1}
% \end{minipage}%
% %\hfill\vline
% \hfill
% \begin{minipage}{0.47\textwidth}
% \begin{align}
% \text{Global phase }  \frac{1}{S} \mathbf{g}_{\eta_{s}} , \pi_{s,t} \mathbf{g}_{\eta_{s}} + \mathbf{d}_{\eta_{s}}
% \end{align}
% % \equationset{Global phase}\label{eqset:2}
% \end{minipage}



In the following, an iteration number $i$





% \begin{lemma}\label{lemma:dist}
% Let $\begin{bmatrix} \mathbf{g}_{\eta_{s,i}} \\ \vdots \\ \mathbf{g}_{\omega_{s,i}} \end{bmatrix} $ be the derivative vector composed of the stochastic derivative w.r.t. the prediction and representation parameters of each data source, where $s \in \{1, \cdots, S\}$.
% $\begin{bmatrix} \pi_{s,i} \mathbf{g}_{\eta_{s,i}} \\ \vdots \\ \pi_{s,i} \mathbf{g}_{\omega_{s,i}} \end{bmatrix}$ represents the corresponding weighted one.
% There exists the following inequality about the distance between the expected gradient vector and the weighted one:
% \begin{align}
% \left\lVert 
% \mathbb{E} \begin{bmatrix} \mathbf{g}_{\eta_{s,i}} \\ \vdots \\ \mathbf{g}_{\omega_{s,i}} \end{bmatrix} 
% - 
% \mathbb{E} \begin{bmatrix} \pi_{s,i} \mathbf{g}_{\eta_{s,i}} \\ \vdots \\ \pi_{s,i} \mathbf{g}_{\omega_{s,i}} \end{bmatrix}
% \right\rVert^2
% \leq 
% \mathbb{E} \left\lVert \begin{bmatrix} \mathbf{g}_{\eta_{s,i}} \\ \vdots \\ \mathbf{g}_{\omega_{s,i}} \end{bmatrix} \right\rVert^2
% \end{align}
% \end{lemma}

% \begin{proof}

% \begin{align}
% \left\lVert 
% \mathbb{E} \begin{bmatrix} \mathbf{g}_{\eta_{s,i}} \\ \vdots \\ \mathbf{g}_{\omega_{s,i}} \end{bmatrix}
% - \mathbb{E} \begin{bmatrix} \pi_{s,i} \mathbf{g}_{\eta_{s,i}} \\ \vdots \\ \pi_{s,i} \mathbf{g}_{\omega_{s,i}} \end{bmatrix}
% \right\rVert^2
% & = 
% \left\lVert 
% \mathbb{E}\begin{bmatrix} (1-\pi_{s,i}) \mathbf{g}_{\eta_{s,i}} \\ \vdots \\ (1-\pi_{s,i}) \mathbf{g}_{\omega_{s,i}} \end{bmatrix}
% \right\rVert^2 \\
% & \leq 
% \mathbb{E}\left\lVert \begin{bmatrix} (1-\pi_{s,i}) \mathbf{g}_{\eta_{s,i}} \\ \vdots \\ (1-\pi_{s,i}) \mathbf{g}_{\omega_{s,i}} \end{bmatrix} \right\rVert^2 \\
% & =
% \mathbb{E}\left[ \sum_{s=1}^S (1-\pi_{s,i})^2 (\norm{\mathbf{g}_{\eta_{s,i}}}^2 + \norm{\mathbf{g}_{\omega_{s,i}}}^2) \right] \\
% & \leq
% \mathbb{E}\left[ \sum_{s=1}^S (\norm{\mathbf{g}_{\eta_{s,i}}}^2 + \norm{\mathbf{g}_{\omega_{s,i}}}^2) \right] \\
% & =
% \mathbb{E} \left\lVert \begin{bmatrix} \mathbf{g}_{\eta_{s,i}} \\ \vdots \\ \mathbf{g}_{\omega_{s,i}} \end{bmatrix} \right\rVert^2
% % = \frac{1}{S} \mathbb{E}[ \norm{\mathring{\mathbf{g}}_i}^2 ]
% \end{align}

% \end{proof}


The following theorem shows the favorable behavior of the overall loss function during the component phase, i.e. it is moving towards (a neighborhood of) a stationary point of all parameters, despite the component phase is focused on learning parts of the parameters.

\begin{theorem}\label{theory:loss_decline}
Assume the loss function $\mathcal{L} \big( \{\eta_{s}, \omega_{s}\}_{s=1}^S, \theta \,;\, \mathcal{D} \big)$ is L-smooth.
For all stochastic derivatives $\mathbf{g} \in \{ \mathbf{g}_{\omega_{1}}, \cdots, \mathbf{g}_{\omega_{S}}, \mathbf{g}_{\eta_{1}}, \cdots, \mathbf{g}_{\eta_{S}}, \mathbf{g}_{\theta} \}$, the stochastic gradient is bounded $\mathbb{E}\lVert \mathbf{g} \rVert^2 \leq G^2$ and the variance is bounded $\mathbb{E} \lVert \mathbf{g} - \mathbb{E}[\mathbf{g}] \rVert^2 \leq \zeta^2$.
In the component phase, for the iteration step $i = 0, \cdots, I$, let $\Theta_i$ represent the entire set of parameters to train, i.e. $\Theta_i = \big\{ \{\eta_{s,i}, \omega_{s,i} \}_{s=1}^S, \theta_{0} \big\}$, where $\theta$ stays at step $0$, since it is not updated in the component phase. 

\tian{$\mu$}
Then, in the component phase, as the parameters $\{\eta_s, \omega_s\}_{s=1}^S$ are updated through minimizing $\overline{\mathcal{L}}\big( \{\eta_s, \omega_s\}_{s=1}^S \big)$, in expectation the overall loss function $\mathcal{L}\left( \{\eta_s, \omega_s\}_{s=1}^S, \theta \right)$ converges towards (a neighborhood of) a stationary point by the following:
\begin{align}
\frac{1}{I+1} \sum_{i=0}^I \mathbb{E}[ \norm{\nabla \mathcal{L}(\Theta_i)}^2 ]  
\leq
\frac{2S\mathbb{E}[\mathcal{L}\left( \Theta_{I} \right)] - \mathbb{E}[\mathcal{L}\left( \Theta_{0} \right)]}{\mu (I+1)} 
+ 2 (S \zeta^2 + S G^2 + \mu L G^2) 
\end{align}
\end{theorem}

The rightmost term in (2) measures the average quality of the pruning. However, unless δt → 0 or
kwtk → 0 for t → ∞, the error term never completely vanishes, meaning that the method converges
only to a neighborhood of the optimal solution (this not only holds for the pruned model, but also for
3Our variable wt corresponds to x˜t in the notation of Karimireddy et al. (2019). Their error-fixed SGD
algorithm evaluates gradients at perturbed iterates xt := x˜t + et, which correspond precisely to w˜ t = wt + et
in our notation. This shows the connection of these two methods.
the jointly maintained dense model, as we will show in the appendix). This behavior is expected, as
the global optimal model w? might be dense and cannot be approximated well by a sparse model.

share version of the model


% \begin{proof}

% it is

% $\mathbf{g}_{\omega_{s,i}} = -\frac{\partial \log p_{\mathbf{\omega}_{s,i}}(y \,|\, z = s, \widetilde{\mathbf{h}}_{s,i})}{\partial \omega_{s,i}} $

% $\mathbf{g}_{\eta_{s,i}} = -\frac{\partial \log p_{\omega_{s,i}}(y \,|\, z = s, \widetilde{\mathbf{h}}_{s,i})}{\partial \widetilde{\mathbf{h}}_{s,i}} \cdot \nabla\widetilde{\mathbf{h}}_{s,i}$

% $\mathbf{d}_{\eta_{s,i}} = \sum_{k=1}^{S} \pi_{k,i} \frac{\partial \log\mathbb{P}_{\theta}(z=k|\cdot)}{\partial \widetilde{\mathbf{h}}_{s,i}} \cdot \nabla\widetilde{\mathbf{h}}_{s,i}$

% $\mathbf{g}_{\theta_{i}} = -\sum_{k=1}^{S} \pi_{k,i}  \frac{\partial \log\mathbb{P}(z=k|\cdot)}{\partial \theta_{i}}$

% % --
% original 

% $ \mathbf{g}_i = \begin{bmatrix} \pi_{s,i} \mathbf{g}_{\eta_{s,i}} + \mathbf{d}_{\eta_{s,i}} \\ \vdots \\ \pi_{s,i} \mathbf{g}_{\omega_{s,i}} \\ \vdots \\ \mathbf{g}_{\theta_{i}} \end{bmatrix} $

% $\nabla \mathcal{L}\left( \{\eta_{s,i}, \omega_{s, i}\}_{s=1}^S, \theta_i \right) = \mathbb{E}[\mathbf{g}_i]$

% % --
% lower bound 

% $\mathbf{\overline{g}}_i = \begin{bmatrix} \frac{1}{S}\mathbf{g}_{\eta_{s,i}} \\ \vdots \\ \frac{1}{S} \mathbf{g}_{\omega_{s,i}} \\ \vdots \\ \mathbf{0} \end{bmatrix}$

% $\nabla \overline{\mathcal{L}} \big( \{\eta_{s,i}, \omega_{s,i}\}_{s=1}^S \big) = \mathbb{E}[\mathbf{\overline{g}}_i]$

% $\mathring{\mathbf{g}}_i = \begin{bmatrix} \mathbf{g}_{\eta_{s,i}} \\ \vdots \\ \mathbf{g}_{\omega_{s,i}} \\ \vdots \\ \mathbf{0} \end{bmatrix}$

% % --
% \begin{align}
% & \mathbb{E}[\mathcal{L}\left( \{\eta_{s,i+1}, \omega_{s,i+1} \}_{s=1}^S, \theta_{i+1} \right)] - \mathbb{E}[\mathcal{L}\left( \{\eta_{s,i}, \omega_{s,i} \}_{s=1}^S, \theta_{i} \right)] \\
% \leq & 
% -\mu \langle \mathbb{E}[\mathbf{\overline{g}}_i], \mathbb{E}[\mathbf{g}_i] \rangle 
% +\frac{\mu^2 L}{2} \mathbb{E}[ \norm{\mathbf{\overline{g}}_i}^2 ] \\
% = & 
% -\frac{\mu}{S} \langle \mathbb{E}[\mathring{\mathbf{g}}_i], \mathbb{E}[\mathbf{g}_i] \rangle
% +\frac{\mu^2 L}{2S^2} \mathbb{E}[ \norm{\mathring{\mathbf{g}}_i}^2 ] \label{eq:theory_1}
% \end{align}

% where h·, ·i is the Euclidean inner product on tensor, dot product of two vectors 

% \begin{align}
% -\frac{\mu}{S} \langle \mathbb{E}[\mathbf{\mathring{g}}_i], \mathbb{E}[\mathbf{g}_i] \rangle = 
%  \frac{\mu}{2S} \big\lVert \mathbb{E}[\mathbf{\mathring{g}}_i] - \mathbb{E}[\mathbf{g}_i] \big\rVert^2
% -\frac{\mu}{2S} \big\lVert \mathbb{E}[\mathbf{\mathring{g}}_i] \big\rVert^2
% -\frac{\mu}{2S} \big\lVert \mathbb{E}[\mathbf{g}_i] \big\rVert^2
% \end{align}

% with $\norm{a+b}^2 \leq 2\norm{a}^2 + 2\norm{b}^2$

% \begin{align}
% \frac{\mu}{2S}\norm{\mathbb{E}[\mathbf{\mathring{g}}_i] - \mathbb{E}[\mathbf{g}_i]}^2 
% & = \frac{\mu}{2S} 
% \left\lVert 
% \mathbb{E}\begin{bmatrix} \mathbf{g}_{\eta_{s,i}} \\ \vdots \\ \mathbf{g}_{\omega_{s,i}} \\ \vdots \\ \mathbf{0} \end{bmatrix}
% - \mathbb{E}\begin{bmatrix} \pi_{s,i} \mathbf{g}_{\eta_{s,i}} + \delta_{\eta_{s,i}} \\ \vdots \\ \pi_{s,i} \mathbf{g}_{\omega_{s,i}} \\ \vdots \\ \mathbf{g}_{\theta_{i}} \end{bmatrix} \right\rVert^2 \\
% & = \frac{\mu}{2S} 
% \left\lVert 
% \mathbb{E}\begin{bmatrix} \mathbf{g}_{\eta_{s,i}} \\ \vdots \\ \mathbf{g}_{\omega_{s,i}} \\ \vdots \\ \mathbf{0} \end{bmatrix}
% - \mathbb{E} \begin{bmatrix} \pi_{s,i} \mathbf{g}_{\eta_{s,i}} \\ \vdots \\ \pi_{s,i} \mathbf{g}_{\omega_{s,i}} \\ \vdots \\ \mathbf{0} \end{bmatrix}  
% - \mathbb{E} \begin{bmatrix} \delta_{\eta_{s,i}} \\ \vdots \\ \mathbf{0} \\ \vdots \\ \mathbf{g}_{\theta_{i}} \end{bmatrix} 
% \right\rVert^2 \\
% & \leq \frac{\mu}{S} 
% \left\lVert 
% \mathbb{E}\begin{bmatrix} \mathbf{g}_{\eta_{s,i}} \\ \vdots \\ \mathbf{g}_{\omega_{s,i}} \\ \vdots \\ \mathbf{0} \end{bmatrix}
% - \mathbb{E} \begin{bmatrix} \pi_{s,i} \mathbf{g}_{\eta_{s,i}} \\ \vdots \\ \pi_{s,i} \mathbf{g}_{\omega_{s,i}} \\ \vdots \\ \mathbf{0} \end{bmatrix}
% \right\rVert^2
% + \frac{\mu}{S} 
% \left\lVert 
% \mathbb{E} \begin{bmatrix} \delta_{\eta_{s,i}} \\ \vdots \\ \mathbf{0} \\ \vdots \\ \mathbf{g}_{\theta_{i}} \end{bmatrix}
% \right\rVert^2
% \end{align}


% \begin{align}
% \frac{\mu}{S} 
% \left\lVert 
% \mathbb{E}\begin{bmatrix} \mathbf{g}_{\eta_{s,i}} \\ \vdots \\ \mathbf{g}_{\omega_{s,i}} \\ \vdots \\ \mathbf{0} \end{bmatrix}
% - \mathbb{E} \begin{bmatrix} \pi_{s,i} \mathbf{g}_{\eta_{s,i}} \\ \vdots \\ \pi_{s,i} \mathbf{g}_{\omega_{s,i}} \\ \vdots \\ \mathbf{0} \end{bmatrix}
% \right\rVert^2 
% \leq 
% \frac{\mu}{S} 
% \mathbb{E}[ \sum_{s=1}^S (\norm{\mathbf{g}_{\eta_{s,i}}}^2 + \norm{\mathbf{g}_{\omega_{s,i}}}^2) ] 
% = \frac{\mu}{S} \mathbb{E}\norm{\mathring{\mathbf{g}}_i}^2
% \end{align}

% assumption

% $\mathbb{E}[ \norm{\mathbf{g}_{\omega_{s,i}}}^2 ]$ $G^2$, $\zeta^2$

% $\mathbb{E}[ \norm{\mathbf{g}_{\eta_{s,i}}}^2 ]$

% $\mathbb{E}[ \norm{\mathbf{\delta}_{\eta_{i}}}^2 ]$

% $\mathbb{E}[ \norm{\mathbf{g}_{\theta_{i}}}^2 ]$

% \begin{align}
% (\ref{eq:theory_1}) 
% & \leq 
% \frac{\mu}{S}\mathbb{E}\norm{\mathring{\mathbf{g}}_i}^2 
% + \frac{\mu}{S} 
% \left\lVert 
% \mathbb{E} \begin{bmatrix} \mathbf{d}_{\eta_{s,i}} \\ \vdots \\ \mathbf{0} \\ \vdots \\ \mathbf{g}_{\theta_{i}} \end{bmatrix}
% \right\rVert^2
% -\frac{\mu}{2S}\norm{ \mathbb{E}[\mathbf{\mathring{g}}_i] }^2
% -\frac{\mu}{2S}\norm{ \mathbb{E}[\mathbf{g}_i] }^2 
% +\frac{\mu^2 L}{2S^2}\mathbb{E} \norm{\mathring{\mathbf{g}}_i}^2 \\
% & \leq
% \frac{\mu}{2S}\mathbb{E}\norm{\mathring{\mathbf{g}}_i}^2 
% + \frac{\mu}{2S}\mathbb{E}\norm{\mathring{\mathbf{g}}_i}^2
% -\frac{\mu}{2S}\norm{ \mathbb{E}[\mathbf{\mathring{g}}_i] }^2
% + \frac{\mu}{S} 
% \left\lVert 
% \mathbb{E} \begin{bmatrix} \mathbf{d}_{\eta_{s,i}} \\ \vdots \\ \mathbf{0} \\ \vdots \\ \mathbf{g}_{\theta_{i}} \end{bmatrix}
% \right\rVert^2
% -\frac{\mu}{2S}\norm{ \mathbb{E}[\mathbf{g}_i] }^2 
% +\frac{\mu^2 L}{2S^2}\mathbb{E} \norm{\mathring{\mathbf{g}}_i}^2 \\
% \end{align}

% \begin{align}
% & \mathbb{E}[\mathcal{L}\left( \{\eta_{s,i+1}, \omega_{s,i+1} \}_{s=1}^S, \theta_{i+1} \right)] - \mathbb{E}[\mathcal{L}\left( \{\eta_{s,i}, \omega_{s,i} \}_{s=1}^S, \theta_{i} \right)] \\
% \leq 
% & \mu\zeta^2 
% + \mu G^2
% -\frac{\mu}{2S}\norm{\mathbb{E}[\mathbf{g}_i]}^2 
% +\frac{\mu^2 L}{S}G^2 
% \end{align}

% \begin{align}
% \frac{1}{I+1} \sum_{i=0}^I \norm{\mathbb{E}[\mathbf{g}_i]}^2 
% \leq
% \frac{2S\mathbb{E}[\mathcal{L}\left( \Theta_{0} \right)] - \mathbb{E}[\mathcal{L}\left( \Theta_{I} \right)]}{\mu (I+1)} 
% + 2 (S \zeta^2 + S G^2 + \mu L G^2) 
% \end{align}

% $ 0 \leq \pi_{s,i} \leq 1$

% Summing these inequalities from t = 0 to t = T gives

% \end{proof}



residual model, representation only through gate

regularization effect





\textbf{Implementation}

\textbf{? partial gradient clipping}

the number of phase epoch fix or as hyper parameter 

prediction interval


------------ proof:

phase 1, bound, distance to original update, variance

% where $\Theta_i$ represents $[\{\eta_{s,i}, \omega_{s,i} \}_{s=1}^S, \theta_{i}]$
% of minimizing the loss function $\mathcal{L}\left( \{\eta_s, \omega_s\}_{s=1}^S, \theta \right)$ or $\mathcal{L}\left( \{\eta_s, \omega_s\}_{s=1}^S, \theta, \{\tau_s\}_{s=1}^S \right)$, 
% n and 
% $\forall \mathbf{g} \in \{ \mathbf{g}_{\omega_{s}}, \mathbf{g}_{\eta_{s}}, \mathbf{g}_{\theta_{i}} \}$  $\mathbb{E}[ \lVert \delta - \mathbb{E}[\delta] \rVert^2]$
% $\mathbb{E} \lVert \delta \rVert^2$
% A function f(x) : R is said to be Lipschitz-smooth with constant L if, f(x) has bounded gradients, 
% mean-squared error of our gradient samples from the
% true gradient is bounded
% Let the learning rate satisfies,
% it holds— in expectation over the stochasticity a
% partial update through the lower bound still make the full gradient of the original loss function converge to 
% Then, following the update of the component specific parameters $\overline{\mathcal{L}}\big( \{\eta_s, \omega_s\}_{s=1}^S \big)$


% The latent variable $z_t$ is a discrete random variable defined on the set of values $\{1, \cdots, S\}$, each of which represents the corresponding data source. The quantity $p_{\theta_s}(y_t | z_t = s, \mathbf{x}_{s, <t})$ models the predictive probabilistic density of the target based on the historical data $\mathbf{x}_{s, <t}$ from a certain source $s$. 
% The quantity\footnote{We indicate with $p_\theta$ probability densities and $\mathbb{P}_{\omega}$ probability mass functions.} $\mathbb{P}_{\omega}(z_t = s \, | \mathbf{x}_{1, <t}, \cdots, \mathbf{x}_{S, <t})$ characterizes a time-varying categorical distribution dependent on multi-source data.
% It adaptively adjusts the contribution of the data source specific density $p_{\theta_s}(y_t | z_t = s, \mathbf{x}_{s, <t})$ at each time step. Clearly, it holds
% $\sum_{s = 1}^{S}\mathbb{P}_{\omega}(z_t = s \, | \mathbf{x}_{1, <t}, \cdots, \mathbf{x}_{S, <t}) = 1$. 
% Finally, $\Theta \triangleq \{ \theta_1, \cdots, \theta_S, \omega \}$ represents the parameters in data source specific components and the latent variable's probability function, and it will be learned in the training phase discussed below. 

% The latent variable $z_t$ is a discrete random variable defined on the set of values $\{1, \cdots, S\}$, each of which represents the corresponding data source. The quantity $p_{\theta}(y_t | z_t = s, \mathbf{x}_{s, <t})$ models the predictive probabilistic density of the target based on the historical data $\mathbf{x}_{s, <t}$ from a certain source $s$. The quantity\footnote{We indicate with $p_\theta$ probability densities and $\mathbb{P}_{\omega}$ probability mass functions.} $\mathbb{P}_{\omega}(z_t = s \, | \mathbf{x}_{1, <t}, \cdots, \mathbf{x}_{S, <t})$ is time-varying dependent on multi-source data and  adaptively adjusts the contribution of the data source specific density $p_{\theta}(y_t | z_t = s, \mathbf{x}_{s, <t})$ at each time step. Clearly, it holds
% $\sum_{s = 1}^{S}\mathbb{P}_{\omega}(z_t = s \, | \mathbf{x}_{1, <t}, \cdots, \mathbf{x}_{S, <t}) = 1$. 
% Finally, $\theta$ and $\omega$ in Eq.~\ref{eq:joint} represent the parameters of the probabilistic functions, which are learned in the training phase discussed below. 



% We now specify in detail the mathematical formulation of each component in the temporal mixture model. The inference process we presented so far does not relies on any specific formulation of the model and thus it is flexible to different specifications. 
% Without loss of generality, we present the following model specification for cryptocurrency data of this paper's interest.

% To specify the model, we need to define the predictive density function of individual sources, i.e. $p_{\theta}(y_t | z_t = s, \mathbf{x}_{s, <t})$ and the probability function of latent variable, i.e. $\mathbb{P}_{\omega}(z_t = s \, | \mathbf{x}_{1, <t}, \cdots, \mathbf{x}_{S, <t})$.
% %In the following learning phase, training instances have to contain data of unified shape. 
% We make a general assumption for both these functions that data from different sources are taken within the same time window w.r.t. the target time step.
% We denote by $h$ the window length, i.e. the number of past time steps which enter in the conditional probabilities. 
% We assume that this value is the same for each source.
% Eq.~\ref{eq:joint} is thus simplified as:
% \begin{align}
% \begin{split}
% \prod_{t}^{}
% \sum_{z_t = 1}^{S}
% & p_{\theta}(y_t | z_t = s, \mathbf{x}_{s, (-h,t)}) \cdot \\
% & \mathbb{P}_{\omega}(z_t = s | \mathbf{x}_{1,  (-h,t)}, \cdots, \mathbf{x}_{S, (-h,t)}), 
% \end{split}
% \end{align}
% where $\mathbf{x}_{s, (-h,t)}$ represents the data from source $s$ within the time window from $t-h$ to $t-1$ and $\mathbf{x}_{s, (-h,t)} \in \mathbb{R}^{d_s \times h}$. 

% First, for $p_{\theta}(y_t | z_t = s, \mathbf{x}_{s, (-h,t)})$,
% we choose the Gaussian distribution.
% Since $\mathbf{x}_{s, (-h,t)} \in \mathbb{R}^{d_s \times h}$ is a matrix, we choose bi-linear regression to parameterize the mean and variance of the Gaussian distribution as follows: 
% \begin{gather}
% y_t | z_t = s, \mathbf{x}_{s,(-h, t)}, ~~~~~\theta \sim \mathcal{N}\big( \mu_s(\mathbf{x}_{s,(-h, t)} \big), \sigma_s^2(\mathbf{x}_{s,(-h, t)})) \\
% \mu_s(\mathbf{x}_{s,(-h, t)}) = L_{\mu, s}^{\top} \cdot \mathbf{x}_{s,(-h, t)} \cdot R_{\mu, s} + b_{\mu, s} \\
% \sigma_s^2(\mathbf{x}_{s,(-h, t)}) =  (L_{\sigma, s}^{\top} \cdot \mathbf{x}_{s,(-h, t)} \cdot R_{\sigma, s} + b_{\sigma, s} )^2,
% \end{gather}
% where $L_{\mu, s}$, $L_{\sigma, s} \in \mathbb{R}^{d_s}$ and $R_{\mu, s}$, $R_{\sigma, s} \in \mathbb{R}^{h}$. $b_{\mu,s}$, while $b_{\sigma,s} \in \mathbb{R}$ are bias terms. 
% %\textcolor{red}{Fabrizios comment from mail about Gaussian.}
% Note that the above parameters are data source specific and then the parameter set $\theta$ can be denoted by $\theta = \{ L_{\mu, s}, L_{\sigma, s}, R_{\mu, s}, R_{\sigma,s}, b_{\mu,s}, b_{\sigma,s} \}_{s=1}^S$.

% As a results, mean and variance on individual data source are defined as: $\mathbb{E}[{y}_{\tau} | \mathbf{x}_{s, <\tau}, \Theta_m] = \mu_s(\mathbf{x}_{s,(-h, t)})$ and
% $\text{Var}({y}_{\tau} | z_t = s, \mathbf{x}_{s, <\tau}, \Theta_m) = \sigma_s^2(\mathbf{x}_{s,(-h, t)})$. 
% Consequently, the mean and uncertainties in the inference phase can be explicitly calculated.

% Second, we choose for $\mathbb{P}_{\omega}(z_t = s | \mathbf{x}_{1,  (-h,t)})$ a multinomial logistic function:

% \begin{equation}\label{formula:softmax}
% \mathbb{P}_{\omega}(z_t = s | \mathbf{x}_{1,  (-h,t)}, \cdots, \mathbf{x}_{S, (-h,t)})=\frac{\exp(\, f(\mathbf{x}_{s, (-h, t)}) \, )}{ \exp( \, \sum_{k=1}^S f(\mathbf{x}_{k, (-h, t)}) \, )},
% \end{equation}

% \begin{equation}
% f(\mathbf{x}) =   L^{\top} \cdot \mathbf{x} \cdot R + b
% \end{equation}
% where $L,R\in {\mathbb R}^{d_s}$ and $b\in {\mathbb R}$ is a bias term 


% As for $p_{\theta_s}(y_t | z_t = s, \mathbf{x}_{s, (-h,t)})$, due to the non-negative nature of the volume in cryptocurrency exchange and its statistical properties~\cite{bauwens2008moments}, we choose the log-normal distribution to model $y_t$ as:

% \begin{align}
%     \ln y_t \, | z_t \text{=} s, \mathbf{x}_{s,(-h, t)} \, \sim \, \mathcal{N}\big( \mu_{t,s}, \sigma_{t,s}^2)
% \end{align}


% In the following, by deriving the conditional variance of the target in the Bayesian mixture manner, 
% we demonstrate that the total variance is decomposed into aleatoric and epistemic uncertainties, which reflect different aspects of the variance of the target ${y}_{\tau}$.


% where $\omega_m$ is from sample $\Theta_m$.
% Eq.~\ref{eq:var} bridges the aleatoric and epistemic uncertainty by the derivation of total variance of ${y}_{\tau}$ in the Bayesian mixture setting.
% The decomposition in Eq.~\ref{eq:var} also
% theoretically demonstrates the relation between total variance and the aleatoric and epistemic uncertainty in Bayesian modeling, namely the total variance is composed of inherent noise and model uncertainty on the target.

% The aleatoric part in Eq.~\ref{eq:var} stems from variance induced from multi-source data. 
% It captures the noise inherent to the target which could depend on $\mathbf{x}_{s, < \tau}$.
% As a comparison, a classical aleatoric uncertainty (or volatility) estimation model, the GARCH, is typically used to estimate the volatility solely with the target time series.
% It has no mechanism to capture the evolving relevance of multi-source data to the aleatoric uncertainty of the target.  

% The epistemic uncertainty on mean in Eq.~\ref{eq:var} accounts for uncertainty in the model parameters i.e. uncertainty which captures our ignorance about which model generated our collected data.
% This uncertainty can be reduced when enough data are available, and is often referred to as model uncertainty.


==> backup/preliminary.tex <==
\section{Multiple market cryptocurrency data}\label{sec:data}

%\tian{Figure 1 is not mentioned anywhere in the text}

%The prices for the crypto assets are obtained from multiple exchanges.
%This provides a snapshot of how this selection of the crypto market is performing overall in one single, easily understandable measure.
%In this cross-market scenario, markets interplay and information flows between market due to the arbitrage.
Our empirical analyses are performed on a sample of data from two exchanges, Bitfinex\footnote{https://www.bitfinex.com} and Bitstamp\footnote{https://www.bitstamp.net}, where Bitcoins can be exchanged with US dollars. These markets work through a limit order book, as many conventional exchanges. The investigated period is June-November 2018. The main analyses are performed on five-minute intervals, thus the length of the investigated time series is $34,346$, since the markets are open $24/7$. %\textcolor{blue}{Nino: having "," in the number 34346 is maybe confusing. I would just use 34346.}
In the Appendix we also show some analyses performed at one minute resolution, raising the number of data points  to $171$k. 

For each of the two markets we consider two types of data: transaction data and limit order book data.

From \textbf{transaction data} we extract the following features for each 5-min interval:
\begin{itemize}
    \item \textit{Buy volume} - in BTC units of executed transactions
    \item \textit{Sell volume} - in BTC units of executed transactions
    \item \textit{Volume imbalance} - absolute difference between buy and sell volume
    \item \textit{Buy transactions} - number of executed transactions on buy side
     \item \textit{Sell transactions} - number of executed transactions on sell side
     \item \textit{Transaction imbalance} - absolute difference between buy and sell number of transactions
\end{itemize}


From \textbf{limit orderbook data} we extract the following features \cite{OB_rev_Porter2013, Lillo2016}, obtained by averaging the one minute variables in each 5-min interval:
\begin{itemize}
    \item \textit{Spread} is the difference between the highest price that a buyer is willing to pay for a BTC (bid) and the lowest price that a seller is willing to accept (ask).  
    \item \textit{Ask volume} is the number of BTCs on the ask side of order book.
     \item \textit{Bid volume} is the number of BTCs on the bid side of order book.
    \item \textit{Imbalance} is the absolute difference between ask and bid volume. 
    %\item \textit{Weighted spread} is the difference between cumulative price over $10\%$ of bid depth and the cumulative price over $10\%$ of ask depth. 
    \item \textit{Ask/bid Slope} is estimated as the volume until $\delta$ price offset from the best ask/bid price.
     $\delta$ is estimated by the bid  price at the order that has at least 1$\%$, 5$\%$ and 10 $\%$ of orders with the highest bid price. 
    \item \textit{Slope imbalance} is the absolute difference between ask and bid slope at different values of price associated to $\delta$. $\delta$ is estimated by the bid  price at the order that has at least 1$\%$, 5$\%$ and 10 $\%$ of orders with the highest bid price.
    \end{itemize}

The target variable $y_t$ that we aim at forecasting is the sum of the two first features of transaction data of the target market, i.e. the sum of buy and sell volume.

In the proposed modeling approaches (described in Section \ref{sec:model}) we consider different sources that at each time can affect the probability distribution of trading volume in the next time interval in a given market. Given the setting presented above, in our analysis, there are $S=4$ sources, namely one for transaction data and one for limit order book data for the two markets. 
We indicate with $\mathbf{x}_{s,t} \in \mathbb{R}^{d_s} $ the data from source $s$ at time step $t$, and ${d_s}$ the dimensionality of source data $s$. Given the list of variables presented above, we have $d_s=6$ when the source is transaction data in any market, while $d_s=13$ for orderbook data.
%Furthermore, at the same time, we will simultaneously observe data at different exchange markets $M_1, ... M_k$. Combinations of data types and different markets uniquely define the source data $s$.

Figure \ref{fig:volume_statistics} shows the average 1-min transaction volume as a function of the time of the day. We observe the lack of a strong intra-daily "U-shape" component, which is instead observed in other asset classes \cite{andersen1997intraday} and used in intraday volume modeling. 
%Additionally, in Appendix Fig \ref{fig:volume_statistics2} we check the same period in 2019 and observe similar empirical regularities. 
%In this paper, we denote the Bitfinex\footnote{https://www.bitfinex.com} source as market 1 and Bitstamp\footnote{https://www.bitstamp.net} as market 2.


